Work Systems Modeling Library

Modeling of work systems occurs for all sorts of reasons. Requirements need to be expressed. A pre-existing situation may need to be charted and analyzed. Early design decisions may be captured using architecture principles. Detailed design may be worked out. We all regard these activities as essentially being forms of modeling. In the work systems modeling library, we consider work system engineering from a modeling perspective. In the field of work system engineering, a whole plethora of modeling methods is available to system engineers and architects. Each of these methods can be used to model some (aspects) of a domain related to an existing and/or a planned work system. The aspects may refer to requirements, architecture, design, processing, data, etc, etc. In other words, these methodes are essentially all intended to model different aspects of work systems and/or their context. The aim of the work systems modeling library (WSML) is to bring together methodical knowledge concerning the modeling of work systems.

==> Citations/1981-Mathiassen-SystemDevelopment.tex <==
%
%
%
L.~{Mathiassen}. %
{\em {Systemudvikling og Systemudviklings--Metode}}. %
PhD thesis, Aarhus University, Aarhus, Denmark, EU, 1981. %
In Danish. %
%
%


==> Citations/1983-Sol-MethodConsideration.tex <==
%
%
%
H.G. {Sol}. %
{A Feature Analysis of Information Systems Design Methodologies: %
Methodological Considerations}. %
In T.W. {Olle}, H.G. {Sol}, and C.J. {Tully}, editors, {\em %
{Information Systems Design Methodologies: A Feature Analysis, Amsterdam, The %
Netherlands, EU}}, pages 1--7. North--Holland/IFIP WG8.1, Amsterdam, The %
Netherlands, EU, 1983. ISBN 0444867058 %
%
%


==> Citations/1984-Kensing-MethodEvaluation.tex <==
%
%
%
F.~{Kensing}. %
{Towards Evaluation of Methods for Property Determination: A %
Framework and a Critique of the Yourdon--DeMarco Approach}. %
In T.M.A. {Bemelmans}, editor, {\em {Beyond Productivity: Information %
Systems Development for Organizational Effectiveness, Amsterdam, The %
Netherlands, EU}}, pages 325--338. North--Holland, Amsterdam, The %
Netherlands, EU, 1984. %
%
%


==> Citations/1985-WoodHarper-Multiview.tex <==
%
%
%
A.T. {Wood--Harper}, L.~{Antill}, and D.E. {Avison}. %
{\em {Information Systems Definition: The Multiview Approach}}. %
Blackwell, Oxford, United Kingdom, EU, 1985. ISBN 0632012168 %
%
%


==> Citations/1987-Zachman-ISA.tex <==
%
%
%
J.A. {Zachman}. %
{A framework for information systems architecture}. %
{\em IBM Systems Journal}, 26(3), 1987. %
%
%


==> Citations/1988-Sol-InfSystDev.tex <==
%
%
%
H.G. {Sol}. %
{Information Systems Development: A Problem Solving Approach}. %
In {\em {Proceedings of 1988 INTEC Symposium Systems Analysis and %
Design: A Research Strategy}}, 1988. %
%
%


==> Citations/1989-McClure-CASE.tex <==
%
%
%
C.L. {McClure}. %
{\em {CASE is Software Automation}}. %
Prentice--Hall, Englewood Cliffs, New Jersey, USA, 1989. ISBN %
0131193309 %
%
%


==> Citations/1989-Seligmann-Framework.tex <==
%
%
%
P.S. {Seligmann}, G.M. {Wijers}, and H.G. {Sol}. %
{Analyzing the Structure of I.S. Methodologies, an alternative %
approach}. %
In R.~{Maes}, editor, {\em {Proceedings of the First Dutch Conference %
on Information Systems}}, 1989. %
%
%


==> Citations/1990-Wijers-Modelling.tex <==
%
%
%
G.M. {Wijers} and H.~{Heijes}. %
{Automated Support of the Modelling Process: A view based on %
experiments with expert information engineers}. %
In B.~{Steinholz}, A.~{S{\o}lvberg}, and L.~{Bergman}, editors, {\em %
{Proceedings of the Second Nordic Conference CAiSE`90 on Advanced Information %
Systems Engineering, Stockholm, Sweden, EU}}, volume 436 of {\em Lecture %
Notes in Computer Science}, pages 88--108, Berlin, Germany, EU, 1990. %
Springer. ISBN 3540526250 %
%
%


==> Citations/1991-ISO-Quality.tex <==
%
%
%
{\em {Software engineering -- Product quality -- Part 1: Quality model}}, 2001. %
ISO/IEC 9126--1:2001.\\\url{http://www.iso.org} %
%
%
%


==> Citations/1993-Tapscott-ParadigmShift.tex <==
%
%
%
D.~{Tapscott} and A.~{Caston}. %
{\em {Paradigm Shift -- The New Promise of Information Technology}}. %
McGraw--Hill, New York, New York, USA, 1993. ASIN 0070628572 %
%
%


==> Citations/1995-Avison-ISDevMeth.tex <==
%
%
%
D.E. {Avison}. %
{\em {Information Systems Development: Methodologies, Techniques and %
Tools}}. %
McGraw--Hill, New York, New York, USA, 2nd edition, 1995. ISBN %
0077092333 %
%
%


==> Citations/1996-ISO-KSP.tex <==
%
%
%
{ISO}. %
{\em {Kwaliteit van softwareprodukten}}. %
ten Hagen {\&} Stam, Den Haag, The Netherlands, EU, 1996. %
In Dutch. ISBN 9026724306 %
%
%


==> Citations/1996-Rolland-MethEng.tex <==
%
%
%
C.~{Rolland} and N.~{Prakash}. %
{A Proposal for Context--Specific Method Engineering}. %
In S.~{Brinkkemper}, K.~{Lyytinen}, and R.J. {Welke}, editors, {\em %
{Proceedings of the IFIP TC8 WG8.1/8.2 Working Conference on Method %
Engineering}}, pages 191--208, London, United Kingdom, EU, August 1996. %
Chapman {\&} Hall. %
%
%


==> Citations/1996-Rossi-MethodEngineering.tex <==
%
%
%
M.~{Rossi} and S.~{Brinkkemper}. %
{Complexity Metrics for System Development Methods and Techniques}. %
{\em Information Systems}, 21(2):209--227, 1996. %
%
%


==> Citations/1999-Alter-WorkSystems.tex <==
%
%
%
S.~{Alter}. %
{A general, yet useful theory of information systems}. %
{\em Communications of the Association for Information Systems}, %
1(13), 1999.\\\url{http://cais.isworld.org/articles/1-13/default.asp} %
%
%
%


==> Citations/1999-Booch-UML.tex <==
%
%
%
G.~{Booch}, J.~{Rumbaugh}, and I.~{Jacobson}. %
{\em {The Unified Modelling Language User Guide}}. %
Addison Wesley, Reading, Massachusetts, USA, 1999. ISBN 0201571684 %
%
%


==> Citations/1999-Franckson-ISPL-Deliverables.tex <==
%
%
%
M.~{Franckson} and T.F. {Verhoef}, editors. %
{\em {Specifying Deliverables}}. %
Information Services Procurement Library. ten Hagen {\&} Stam, Den %
Haag, The Netherlands, EU, 1999. ISBN 9076304823 %
%
%


==> Citations/1999-IEEE-Architecture.tex <==
%
%
%
{Recommended Practice for Architectural Description of Software Intensive %
Systems}. %
Technical Report IEEE P1471--2000, The Architecture Working Group of %
the Software Engineering Committee, Standards Department, IEEE, Piscataway, %
New Jersey, USA, September 2000. ISBN 0738125180\\\url{http://www.ieee.org} %
%
%
%


==> Citations/1999-Proper-ISPL-LSM.tex <==
%
%
%
H.A.~(Erik) {Proper}, editor. %
{\em {ISP for Large--scale Migrations}}. %
Information Services Procurement Library. ten Hagen {\&} Stam, Den %
Haag, The Netherlands, EU, 2001. ISBN 9076304882 %
%
%


==> Citations/2000-Proper-ISEBOK.tex <==
%
%
%
H.A.~(Erik) {Proper}, H.~{Bosma}, S.J.B.A. {Hoppenbrouwers}, and R.D.T. %
{Janssen}. %
{Towards an Information Systems Engineering Body of Knowledge}. %
In D.B.B. {Rijsenbrij}, editor, {\em {Proceedings of the Second %
National Architecture Congres}}, November 2000. %
%
%


==> Citations/2001-Halpin-ORM.tex <==
%
%
%
T.A. {Halpin}. %
{\em {Information Modeling and Relational Databases, From Conceptual %
Analysis to Logical Design}}. %
Morgan Kaufmann, San Mateo, California, USA, 2001. ISBN 1558606726 %
%
%


==> Citations/2001-Janssen-AML.tex <==
%
%
%
R.D.T. {Janssen}, H.A.~(Erik) {Proper}, H.~{Bosma}, D.~{Verhoef}, and S.J.B.A. %
{Hoppenbrouwers}. %
{Developing an Architecture Method Library}. %
Technical report, Ordina Institute, Gouda, The Netherlands, EU, %
January 2001. %
%
%


==> Citations/2002-Alter-WorkSystems.tex <==
%
%
%
S.~{Alter}. %
{The work system method for understanding information systems and %
information system research}. %
{\em Communications of the Association for Information Systems}, %
9(9):90--104, %
2002.\\\url{http://cais.isworld.org/articles/default.asp?vol=9&art=6} %
%
%
%


==> Citations/2002-Heuvel-ArchitectuurPragmatiek.tex <==
%
%
%
W.-J. van~den {Heuvel} and H.A.~(Erik) {Proper}. %
{De pragmatiek van Architectuur}. %
{\em Informatie}, 44(11):12--14, 2002. %
In Dutch. %
%
%


==> Citations/2003-Greefhorst-Frameworks.tex <==
%
%
%
D.~{Greefhorst}, H.~{Koning}, and H.~van {Vliet}. %
{Dimensies in raamwerken}. %
{\em Informatie}, 45(11):22--27, 2003. %
In Dutch. %
%
%


==> Citations/2004-Proper-DaVinci.tex <==
%
%
%
H.A.~(Erik) {Proper}. %
{\em {Architecture--driven Information Systems Engineering}}. %
DaVinci Series. Nijmegen Institute for Information and Computing %
Sciences, University of Nijmegen, Nijmegen, The Netherlands, EU, 2004. %
%
%


==> Citations/2005-Lankhorst-ArchiMate.tex <==
%
%
%
M.M. {Lankhorst} and {others}. %
{\em {Enterprise Architecture at Work: Modelling, Communication and %
Analysis}}. %
Springer, Berlin, Germany, EU, 2005. ISBN 3540243712 %
%
%


==> Citations/2005-Proper-CommunicatingArchitecture.tex <==
%
%
%
H.A.~(Erik) {Proper}, S.J.B.A. {Hoppenbrouwers}, and G.E. {Veldhuijzen van %
Zanten}. %
{Communication of Enterprise Architectures}. %
In M.M. {Lankhorst}, editor, {\em {Enterprise Architecture at Work: %
Modelling, Communication and Analysis, Berlin, Germany, EU}}, pages 67--82. %
Springer, Berlin, Germany, EU, 2005. ISBN 3540243712 %
%
%


==> Citations/2005-Proper-DaVinciOverview.tex <==
%
%
%
H.A.~(Erik) {Proper}. %
{\em {An Overview of the DaVinci Series}}. %
DaVinci Series. Nijmegen Institute for Information and Computing %
Sciences, University of Nijmegen, Nijmegen, The Netherlands, EU, 2005. %
%
%


==> definitions/100-percent-principle/def.tex <==
The \DefinitionName{information-grammar}{ls} should describe 
\emph{precisely all} conceptual aspects.


==> definitions/100-percent-principle/lp.tex <==
100\% Principle%


==> definitions/100-percent-principle/ls.tex <==
100\% Principle%


==> definitions/100-percent-principle/up.tex <==
100\% Principle%


==> definitions/100-percent-principle/us.tex <==
100\% Principle%


==> definitions/WSML/def.tex <==
Abbreviation for \DefinitionName{work-system}{ls} 
\DefinitionName{modeling}{ls} library. A library of methodical \DefinitionName{knowledge}{ls} pertaining to the 
\DefinitionName{modeling}{ls} of \DefinitionName{work-system}{lp}.


==> definitions/WSML/lp.tex <==
WSMLs%


==> definitions/WSML/ls.tex <==
WSML%


==> definitions/WSML/up.tex <==
WSMLs%


==> definitions/WSML/us.tex <==
WSML%


==> definitions/abstraction/def.tex <==
Omitting unessential details.


==> definitions/abstraction/lp.tex <==
abstractions%


==> definitions/abstraction/ls.tex <==
abstraction%


==> definitions/abstraction/up.tex <==
Abstractions%


==> definitions/abstraction/us.tex <==
Abstraction%


==> definitions/action-oriented/def.tex <==
The action-oriented \DefinitionName{approach}{ls} interprets sentences 
as events occurring in the \DefinitionName{uod}{ls}. This 
\DefinitionName{approach}{ls} is when the operations on the 
\DefinitionName{data}{ls} are dominant. See also 
\DefinitionName{fact-oriented}{ls}.


==> definitions/action-oriented/lp.tex <==
action oriented%


==> definitions/action-oriented/ls.tex <==
action oriented%


==> definitions/action-oriented/up.tex <==
Action oriented%


==> definitions/action-oriented/us.tex <==
Action oriented%


==> definitions/active-system/def.tex <==
A special kind of \DefinitionName{system}{ls} that is conceived of as 
begin able to change parts of the \DefinitionName{universe}{ls}.


==> definitions/active-system/lp.tex <==
active systems%


==> definitions/active-system/ls.tex <==
active system%


==> definitions/active-system/up.tex <==
Active systems%


==> definitions/active-system/us.tex <==
Active system%


==> definitions/activity-participation/def.tex <==
A \DefinitionName{system-link}{ls} between a 
\DefinitionName{system-activity}{ls} and one of its 
\DefinitionName{actor}{ls}.


==> definitions/activity-participation/lp.tex <==
activity participations%


==> definitions/activity-participation/ls.tex <==
activity participation%


==> definitions/activity-participation/up.tex <==
Activity participations%


==> definitions/activity-participation/us.tex <==
Activity participation%


==> definitions/actor/def.tex <==
A \DN{system-element} that is conceived of as having some involvement in a
\DN{system-activity}. This involvement is a special kind of
\DN{system-link}, referred to as an \DN{activity-participation}.


==> definitions/actor/lp.tex <==
actors%


==> definitions/actor/ls.tex <==
actor%


==> definitions/actor/up.tex <==
Actors%


==> definitions/actor/us.tex <==
Actor%


==> definitions/agens/def.tex <==
The role in a sentence that most commonly is associated with the 
grammatical subject.


==> definitions/agens/lp.tex <==
agens%


==> definitions/agens/ls.tex <==
agens%


==> definitions/agens/up.tex <==
Agens%


==> definitions/agens/us.tex <==
Agens%


==> definitions/alignment/def.tex <==
A \DN{system} $S_1$ is aligned to a system $S_2$ if, and only if, system $S_1$ meets {\em all} \PDN{requirement} posed by $S_2$ on $S_1$.

This alignment may be strived for at different levels of refinement of a system design.


==> definitions/alignment/lp.tex <==
alignment%


==> definitions/alignment/ls.tex <==
alignment%


==> definitions/alignment/up.tex <==
Alignment%


==> definitions/alignment/us.tex <==
Alignment%


==> definitions/application-domain/def.tex <==
That part of the world around is that is to be modelled in the context 
of the development of some application. See also 
\DefinitionName{uod}{ls}.


==> definitions/application-domain/lp.tex <==
application domains%


==> definitions/application-domain/ls.tex <==
application domains%


==> definitions/application-domain/up.tex <==
Application domains%


==> definitions/application-domain/us.tex <==
Application domain%


==> definitions/approach/def.tex <==
\Synonym{way-of-working}


==> definitions/approach/lp.tex <==
approaches%


==> definitions/approach/ls.tex <==
approach%


==> definitions/approach/up.tex <==
Approaches%


==> definitions/approach/us.tex <==
Approach%


==> definitions/architecting/def.tex <==
The processes which tie \DN{definition}, \DN{design} and \DN{deployment} and
to the explicit and implicit needs, desires and requirements
of the usage context. Issues such as: business/IT alignment, stakeholders,
limiting design freedom, negotiation between stakeholders, enterprise
architectures, stakeholder communication, and outsourcing, typify these
processes. 


==> definitions/architecting/lp.tex <==
architecting%


==> definitions/architecting/ls.tex <==
architecting%


==> definitions/architecting/up.tex <==
Architecting%


==> definitions/architecting/us.tex <==
Architecting%


==> definitions/architectural-description/def.tex <==
A \DN{system-description} documenting/describing an \DN{architecture}.


==> definitions/architectural-description/lp.tex <==
architectural descriptions%


==> definitions/architectural-description/ls.tex <==
architectural description%


==> definitions/architectural-description/up.tex <==
Architectural descriptions%


==> definitions/architectural-description/us.tex <==
Architectural description%


==> definitions/architecture-driven-information-system-engineering/def.tex <==
\UDN{information-system-engineering}, using \DN{architecture} as a means to
\begin{itemize}
   \item guide \& control the design and evolution of the \DN{information-system},
   \item evaluate \& compare different information system alternatives, 
   \item negotiate the \PDN{concern} of the information system's \PDN{stakeholder},
\end{itemize}
with the aim of optimising the \DN{alignment} of the resulting
information system to its relevant, technological, organisation and human context (systems).


==> definitions/architecture-driven-information-system-engineering/lp.tex <==
architecture-driven information system engineering%


==> definitions/architecture-driven-information-system-engineering/ls.tex <==
architecture-driven information system engineering%


==> definitions/architecture-driven-information-system-engineering/up.tex <==
Architecture-driven information system engineering%


==> definitions/architecture-driven-information-system-engineering/us.tex <==
Architecture-driven information system engineering%


==> definitions/architecture-driven-system-engineering/def.tex <==
\UDN{system-engineering}, using \DN{architecture} as a means to
\begin{itemize}
   \item guide \& control the design and evolution of the \DN{system},
   \item evaluate \& compare different information system alternatives,
   \item negotiate the \PDN{concern} of the information system's \PDN{stakeholder},
\end{itemize}
with the aim of optimising the \DN{alignment} of the resulting
information system to its relevant, technological, organisation and human context (systems).



==> definitions/architecture-driven-system-engineering/lp.tex <==
architecture-driven-system-engineering%


==> definitions/architecture-driven-system-engineering/ls.tex <==
architecture-driven-system-engineering%


==> definitions/architecture-driven-system-engineering/up.tex <==
Architecture-driven-system-engineering%


==> definitions/architecture-driven-system-engineering/us.tex <==
Architecture-driven system engineering%


==> definitions/architecture-principle/def.tex <==
A \DN{design-principle} which is used to direct the design/architecting of
an \DN{architecture}.


==> definitions/architecture-principle/lp.tex <==
architecture principles%


==> definitions/architecture-principle/ls.tex <==
architecture principle%


==> definitions/architecture-principle/up.tex <==
Architecture principles%


==> definitions/architecture-principle/us.tex <==
Architecture principle%


==> definitions/architecture/def.tex <==
A \DN{model} of which the \DN{system-description}, the so-called
\DN{architectural-description}, is used during \DN{system-engineering} to:
    \begin{itemize}
      \item express the fundamental organization of the \DN{system-domain} in 
    terms of \PDN{component}, their relationships to each other and 
    to the \DN{environment} and 
      \item the principles guiding its evolution and design,
    \end{itemize}
    and which's explicit intend is to be used as a means:
    \begin{itemize}
      \item of communication \& negotiation among stakeholders,
      \item to evaluate and compare design alternatives,
      \item to plan, manage, and execute further system development,
      \item to verify the compliance of a system implementation's.
    \end{itemize}
  


==> definitions/architecture/lp.tex <==
architectures%


==> definitions/architecture/ls.tex <==
architecture%


==> definitions/architecture/up.tex <==
Architectures%


==> definitions/architecture/us.tex <==
Architecture%


==> definitions/aspect-system/def.tex <==
an aspect-system $S'$ of a \DN{system} $S$, is a \DN{sub-system}, where the set
of \PDN{model-link} in $S'$ is a proper subset of the set of the
\PDN{link} in $S$.


==> definitions/aspect-system/lp.tex <==
aspect systems%


==> definitions/aspect-system/ls.tex <==
aspect system%


==> definitions/aspect-system/up.tex <==
Aspect systems%


==> definitions/aspect-system/us.tex <==
Aspect system%


==> definitions/atomic-viewpoint/def.tex <==
A \DefinitionName{viewpoint}{ls} which is not decomposed into smaller 
\DefinitionName{viewpoint}{lp}. An \DefinitionName{atomic-viewpoint}{ls} is required to have a one-on-one 
correspondence to a \DefinitionName{way-of-modeling}{ls}/\DefinitionName{technique}{ls} 
that should be used to create \DefinitionName{model}{lp} conforming to this \DefinitionName{viewpoint}{ls}.


==> definitions/atomic-viewpoint/lp.tex <==
atomic viewpoints%


==> definitions/atomic-viewpoint/ls.tex <==
atomic viewpoint%


==> definitions/atomic-viewpoint/up.tex <==
Atomic viewpoints%


==> definitions/atomic-viewpoint/us.tex <==
Atomic viewpoint%


==> definitions/autonomous-system/def.tex <==
an \DN{open-active-system} (possibly also a \DN{responsive-system}, but not a
\DN{reactive-system}) where at least one expression is an action.  A human
being and most (if not all) \PDN{organization} can be regarded as 
\PDN{autonomous-system}.



==> definitions/autonomous-system/lp.tex <==
autonomous systems%


==> definitions/autonomous-system/ls.tex <==
autonomous system%


==> definitions/autonomous-system/up.tex <==
Autonomous systems%


==> definitions/autonomous-system/us.tex <==
Autonomous system%


==> definitions/characterization-dimension/def.tex <==
A set of (possibly ordered) values by which an artefact may be 
characterized.


==> definitions/characterization-dimension/lp.tex <==
characterization dimensions%


==> definitions/characterization-dimension/ls.tex <==
characterization dimension%


==> definitions/characterization-dimension/up.tex <==
Characterization dimensions%


==> definitions/characterization-dimension/us.tex <==
Characterization dimension%


==> definitions/characterization-property/lp.tex <==
characterization properties%


==> definitions/characterization-property/ls.tex <==
characterization property%


==> definitions/characterization-property/up.tex <==
Characterization properties%


==> definitions/characterization-property/us.tex <==
Characterization property%


==> definitions/closed-world-assumption/def.tex <==
All facts not stored in an \DefinitionName{information-system}{ls} are 
assumed to be false. Not that this requires facts with 
\DefinitionName{complete-knowledge}{ls}.


==> definitions/closed-world-assumption/lp.tex <==
closed world assumptions%


==> definitions/closed-world-assumption/ls.tex <==
closed world assumption%


==> definitions/closed-world-assumption/up.tex <==
Closed world assumptions%


==> definitions/closed-world-assumption/us.tex <==
Closed world assumption%


==> definitions/communication/def.tex <==
An exchange of \PDN{message}, i.e.\ a sequence of mutual and alternating
message transfers between at least two \PDN{human-actor}, called communication
partners, whereby these \PDN{message} represent some \DN{knowledge} and are
expressed in languages understood by all communication partners, and whereby
some amount of \DN{knowledge} about the domain of communication and about the
action context and the goal of the communication is made present in all
communication partners.



==> definitions/communication/lp.tex <==
communications%


==> definitions/communication/ls.tex <==
communication%


==> definitions/communication/up.tex <==
Communications%


==> definitions/communication/us.tex <==
Communication%


==> definitions/complete-knowledge/def.tex <==
The value \emph{undefined} is not allowed.


==> definitions/complete-knowledge/lp.tex <==
complete knowledge%


==> definitions/complete-knowledge/ls.tex <==
complete knowledge%


==> definitions/complete-knowledge/up.tex <==
Complete knowledge%


==> definitions/complete-knowledge/us.tex <==
Complete knowledge%


==> definitions/component-system/def.tex <==
A component-system $S'$ of a \DN{system} $S$, is a \DN{sub-system},  where the
set of \PDN{model-concept} in $S'$ is a proper subset of the set of entities in
$S$.


==> definitions/component-system/lp.tex <==
component systems%


==> definitions/component-system/ls.tex <==
component system%


==> definitions/component-system/up.tex <==
Component systems%


==> definitions/component-system/us.tex <==
Component system%


==> definitions/component/def.tex <==
\AbbreviationOf{component-system}



==> definitions/component/lp.tex <==
components%


==> definitions/component/ls.tex <==
component%


==> definitions/component/up.tex <==
Components%


==> definitions/component/us.tex <==
Component%


==> definitions/computerized-information-system/lp.tex <==
computerized information systems%


==> definitions/computerized-information-system/ls.tex <==
computerized information system%


==> definitions/computerized-information-system/up.tex <==
Computerized information systems%


==> definitions/computerized-information-system/us.tex <==
Computerized information system%


==> definitions/concept/def.tex <==
Any \DN{element} from a \DN{conception} that is not a \PDN{link}.


==> definitions/concept/lp.tex <==
concepts%


==> definitions/concept/ls.tex <==
concept%


==> definitions/concept/up.tex <==
Concepts%


==> definitions/concept/us.tex <==
Concept%


==> definitions/conception-evolution/def.tex <==
The evolution of a \DN{conception}.


==> definitions/conception-evolution/lp.tex <==
conception evolutions%


==> definitions/conception-evolution/ls.tex <==
conception evolution%


==> definitions/conception-evolution/up.tex <==
Conception evolutions%


==> definitions/conception-evolution/us.tex <==
Conception evolution%


==> definitions/conception/def.tex <==
That what results, in the mind of a \DN{viewer}, when they interpret a
\DN{perception} of a \DN{domain}.


==> definitions/conception/lp.tex <==
conceptions%


==> definitions/conception/ls.tex <==
conception%


==> definitions/conception/up.tex <==
Conceptions%


==> definitions/conception/us.tex <==
Conception%


==> definitions/conceptualization-principle/def.tex <==
The \DefinitionName{information-grammar}{ls} should not describe any 
does \emph{not} provide any realization (implementation) aspect.


==> definitions/conceptualization-principle/lp.tex <==
Conceptualization principle%


==> definitions/conceptualization-principle/ls.tex <==
conceptualization principle%


==> definitions/conceptualization-principle/up.tex <==
Conceptualization principle%


==> definitions/conceptualization-principle/us.tex <==
Conceptualization principle%


==> definitions/concern/def.tex <==
A \DN{stakeholder}'s interest in properties of a system, relative to
their \PDN{stakeholder-goal}s and the potential role played by the \DN{system}
in achieving these goals. This usually pertains to the system's development,
its operation or any other aspects that are critical or otherwise important to
one or more stakeholders. 


==> definitions/concern/lp.tex <==
concerns%


==> definitions/concern/ls.tex <==
concern%


==> definitions/concern/up.tex <==
Concerns%


==> definitions/concern/us.tex <==
Concern%


==> definitions/construction-process/def.tex <==
A process aiming to realize and test a \DN{system} that is regarded
as a (possibly artificial) artifact that is not yet in operation.


==> definitions/construction-process/lp.tex <==
construction processes%


==> definitions/construction-process/ls.tex <==
construction process%


==> definitions/construction-process/up.tex <==
Construction processes%


==> definitions/construction-process/us.tex <==
Construction process%


==> definitions/construction/def.tex <==
\AbbreviationOf{construction-process}


==> definitions/construction/lp.tex <==
constructions%


==> definitions/construction/ls.tex <==
construction%


==> definitions/construction/up.tex <==
Constructions%


==> definitions/construction/us.tex <==
Construction%


==> definitions/controlled-language/def.tex <==
A \DefinitionName{controlled-language}{ls} is a form of language with 
special restrictions on grammar, style, and vocabulary usage, close to 
natural language, but with a formal base. The objective of a 
\DefinitionName{controlled-language}{ls} is to improve the consistency, 
readability, translatability, and retrievability of 
\DefinitionName{information}{ls}.


==> definitions/controlled-language/lp.tex <==
controlled languages%


==> definitions/controlled-language/ls.tex <==
controlled language%


==> definitions/controlled-language/up.tex <==
Controlled languages%


==> definitions/controlled-language/us.tex <==
Controlled language%


==> definitions/data/def.tex <==
Any representation in some language. Data is therefore simply a collection of
symbols that may, or may not, have some meaning to some \DN{actor}.


==> definitions/data/lp.tex <==
data%


==> definitions/data/ls.tex <==
data%


==> definitions/data/up.tex <==
Data%


==> definitions/data/us.tex <==
Data%


==> definitions/decomposer/def.tex <==
The \DN{link} between a composed \DN{concept} and one of its underlying \PDN{concept}.


==> definitions/decomposer/lp.tex <==
decomposers%


==> definitions/decomposer/ls.tex <==
decomposer%


==> definitions/decomposer/up.tex <==
Decomposers%


==> definitions/decomposer/us.tex <==
Decomposer%


==> definitions/deep-sentence-structure/def.tex <==
Sentences with the same meaning may have distinct surface forms. These 
are derived from an unobservable common source, the so-called deep 
structure underlying both sentences.


==> definitions/deep-sentence-structure/lp.tex <==
deep sentence structures%


==> definitions/deep-sentence-structure/ls.tex <==
deep sentence structure%


==> definitions/deep-sentence-structure/up.tex <==
Deep sentence structures%


==> definitions/deep-sentence-structure/us.tex <==
Deep sentence structure%


==> definitions/definition-description/def.tex <==
The \DefinitionName{description}{ls} of a 
\DefinitionName{definition}{ls}.


==> definitions/definition-description/lp.tex <==
definition descriptions%


==> definitions/definition-description/ls.tex <==
definition description%


==> definitions/definition-description/up.tex <==
Definition descriptions%


==> definitions/definition-description/us.tex <==
Definition description%


==> definitions/definition-process/def.tex <==
A process aiming to identify all requirements that should be
met by the \DN{system} and the \DN{system-description}.

In literature this process may also be referred to as requirements engineering.


==> definitions/definition-process/lp.tex <==
definition processes%


==> definitions/definition-process/ls.tex <==
definition process%


==> definitions/definition-process/up.tex <==
Definition processes%


==> definitions/definition-process/us.tex <==
Definition process%


==> definitions/definition/def.tex <==
The description of the requirements that should be met by both the desired
information system as well as the documents documenting this information
system.  In literature this is also referred to as requirements engineering.

With regards to the information system, the resulting descriptions should
identify: \emph{what} it should do, \emph{how well} it should do this, and
\emph{why} it should do so. With regards to the documentation of 
the information system, the descriptions should identify \emph{what} should be
documented, \emph{how well} it should be documented, and
\emph{why}/\emph{what-for} these documents are needed.  


==> definitions/definition/lp.tex <==
definitions%


==> definitions/definition/ls.tex <==
definition%


==> definitions/definition/up.tex <==
Definitions%


==> definitions/definition/us.tex <==
Definition%


==> definitions/deployment-process/def.tex <==
A process aiming to make a \DefinitionName{system}{ls} operational, 
i.e.\ to implement the use of the \DefinitionName{system}{ls} by its 
prospective users.


==> definitions/deployment-process/lp.tex <==
deployment processes%


==> definitions/deployment-process/ls.tex <==
deployment process%


==> definitions/deployment-process/up.tex <==
Deployment processes%


==> definitions/deployment-process/us.tex <==
Deployment process%


==> definitions/deployment/def.tex <==
The processes of delevering/implementating an information system to/in its
usage context. The \DN{design} of an information system is not enough to arrive
at an operational system. It needs to be implemented-in/delivered-to a usage
context.


==> definitions/deployment/lp.tex <==
deployments%


==> definitions/deployment/ls.tex <==
deployment%


==> definitions/deployment/up.tex <==
Deployments%


==> definitions/deployment/us.tex <==
Deployment%


==> definitions/description-process/def.tex <==
The combination of the \DN{definition-process} and \DN{design-process}.


==> definitions/description-process/lp.tex <==
description processes%


==> definitions/description-process/ls.tex <==
description process%


==> definitions/description-process/up.tex <==
Description processes%


==> definitions/description-process/us.tex <==
Description process%


==> definitions/description/def.tex <==
The result of a \DN{viewer} denoting a \DN{conception}, using some language to
express themselves.



==> definitions/description/lp.tex <==
descriptions%


==> definitions/description/ls.tex <==
description%


==> definitions/description/up.tex <==
Descriptions%


==> definitions/description/us.tex <==
Description%


==> definitions/design-description/def.tex <==
The \DefinitionName{description}{ls} of a \DefinitionName{design}{ls}.


==> definitions/design-description/lp.tex <==
design descriptions%


==> definitions/design-description/ls.tex <==
design description%


==> definitions/design-description/up.tex <==
Design descriptions%


==> definitions/design-description/us.tex <==
Design description%


==> definitions/design-principle/def.tex <==
A system description language, which is intended to aid in the transition from
requirements to design.

Each principle is a predicate over the products of the design process, where a
system is no longer treated as a black-box.  It thus provides direction to the
ensuing design process.


==> definitions/design-principle/lp.tex <==
design principles%


==> definitions/design-principle/ls.tex <==
design principle%


==> definitions/design-principle/up.tex <==
Design principles%


==> definitions/design-principle/us.tex <==
Design principle%


==> definitions/design-process/def.tex <==
A process aiming to design a \DN{system} conform stated requirements.
The resulting system design may range from high-level designs, such
as an strategy or an \DN{architecture}, to the detailed level of 
programming statements or specific worker tasks.



==> definitions/design-process/lp.tex <==
design processes%


==> definitions/design-process/ls.tex <==
design process%


==> definitions/design-process/up.tex <==
Design processes%


==> definitions/design-process/us.tex <==
Design process%


==> definitions/design/def.tex <==
The description of the design of \DN{system}.  These descriptions should
identify \emph{how} an \DN{system} will meet the requirements set out in its
definition.  The resulting design may (depending on the design goals) range
from high-level designs to the detailed level of programming statements or
specific worker tasks.


==> definitions/design/lp.tex <==
designs%


==> definitions/design/ls.tex <==
design%


==> definitions/design/up.tex <==
Designs%


==> definitions/design/us.tex <==
Design%


==> definitions/domain-evolution/def.tex <==
The evolution of a \DN{domain} over time.


==> definitions/domain-evolution/lp.tex <==
domain evolutions%


==> definitions/domain-evolution/ls.tex <==
domain evolution%


==> definitions/domain-evolution/up.tex <==
Domain evolutions%


==> definitions/domain-evolution/us.tex <==
Domain evolution%


==> definitions/domain-expert/def.tex <==
A person that can reveal and assign meaning to statements about the 
\DefinitionName{uod}{ls}. The \DefinitionName{domain-expert}{ls} role 
is further divided into an \DefinitionName{informant}{ls} and a 
\DefinitionName{modeling-mediator}{ls}.


==> definitions/domain-expert/lp.tex <==
domain experts%


==> definitions/domain-expert/ls.tex <==
domain expert%


==> definitions/domain-expert/up.tex <==
Domain experts%


==> definitions/domain-expert/us.tex <==
Falsification%


==> definitions/domain-modeling/def.tex <==
Modeling of the domains that are relevant to the information system being
developed. The resulting models will typically correspond to \emph{ontologies}
of the domains.  These domains can pertain to the information that will be
processed by the information system, the processes in which the information
system will play a role, the processing as it will occur inside the information
system, etc.  Understanding (and modeling) these domains is fundamental to the
other activities in information system engineering.



==> definitions/domain-modeling/lp.tex <==
domain modeling%


==> definitions/domain-modeling/ls.tex <==
domain modeling%


==> definitions/domain-modeling/up.tex <==
Domain modeling%


==> definitions/domain-modeling/us.tex <==
Domain modeling%


==> definitions/domain/def.tex <==
Any `part' or `aspect' of the \DN{universe} a \DN{viewer} may have an \DN{interest} in.


==> definitions/domain/lp.tex <==
domains%


==> definitions/domain/ls.tex <==
domain%


==> definitions/domain/up.tex <==
Domains%


==> definitions/domain/us.tex <==
Domain%


==> definitions/dynamic-system/def.tex <==
A special kind of \DN{system} that is conceived of as undergoing change in the
cause of time.


==> definitions/dynamic-system/lp.tex <==
dynamic systems%


==> definitions/dynamic-system/ls.tex <==
dynamic system%


==> definitions/dynamic-system/up.tex <==
Dynamic systems%


==> definitions/dynamic-system/us.tex <==
Dynamic system%


==> definitions/efficiency/lp.tex <==
efficiency%


==> definitions/efficiency/ls.tex <==
efficiency%


==> definitions/efficiency/up.tex <==
Efficiency%


==> definitions/efficiency/us.tex <==
Efficiency%


==> definitions/element-evolution/def.tex <==
The evolution over time of an \DN{element} in the \DN{conception} of a \DN{viewer}.


==> definitions/element-evolution/lp.tex <==
element evolutions%


==> definitions/element-evolution/ls.tex <==
element evolution%


==> definitions/element-evolution/up.tex <==
Element evolutions%


==> definitions/element-evolution/us.tex <==
Element evolution%


==> definitions/element-version/def.tex <==
The version of an \DN{element-evolution} as it holds at some point in time.
This version is an \DN{element} from a \DN{viewer}'s \DN{conception} of a
\DN{universe}.


==> definitions/element-version/lp.tex <==
element versions%


==> definitions/element-version/ls.tex <==
element version%


==> definitions/element-version/up.tex <==
Element versions%


==> definitions/element-version/us.tex <==
Element version%


==> definitions/element/def.tex <==
The elementary parts of a \DN{viewer}'s \DN{conception}.


==> definitions/element/lp.tex <==
elements%


==> definitions/element/ls.tex <==
element%


==> definitions/element/up.tex <==
Elements%


==> definitions/element/us.tex <==
Element%


==> definitions/elementary-sentence/def.tex <==
Sentences that can not be split into smaller sentences without losing 
\DefinitionName{information}{ls}.


==> definitions/elementary-sentence/lp.tex <==
elementary sentences%


==> definitions/elementary-sentence/ls.tex <==
elementary sentence%


==> definitions/elementary-sentence/up.tex <==
Elementary sentences%


==> definitions/elementary-sentence/us.tex <==
Elementary sentence%


==> definitions/elicitation/def.tex <==
The activity in which the \DefinitionName{system-analyst}{ls} tries to 
obtain sample sentences form the \DefinitionName{domain-expert}{ls}.


==> definitions/elicitation/lp.tex <==
elicitation%


==> definitions/elicitation/ls.tex <==
elicitation%


==> definitions/elicitation/up.tex <==
Elicitation%


==> definitions/elicitation/us.tex <==
Elicitation%


==> definitions/engineering-time-requirement/def.tex <==
A \DN{product-requirement} on any of the products, pertaining to a
\DN{system-engineering} process, other than the resulting system.

These requirements usually refer to \PDN{quality-attribute} such as:
\DN{maintainability} and \DN{portability}.


==> definitions/engineering-time-requirement/lp.tex <==
engineering-time requirements%


==> definitions/engineering-time-requirement/ls.tex <==
engineering-time requirement%


==> definitions/engineering-time-requirement/up.tex <==
Engineering-time requirements%


==> definitions/engineering-time-requirement/us.tex <==
Engineering-time requirement%


==> definitions/enterprise-engineering/def.tex <==
A \DN{system-engineering} process aimed at the creation of an \DN{enterprise-system}.


==> definitions/enterprise-engineering/lp.tex <==
enterprise engineering%


==> definitions/enterprise-engineering/ls.tex <==
enterprise engineering%


==> definitions/enterprise-engineering/up.tex <==
Enterprise engineering%


==> definitions/enterprise-engineering/us.tex <==
Enterprise engineering%


==> definitions/enterprise-system/def.tex <==
An \DN{enterprise}, being a \DN{work-system}, and/or one of its \PDN{sub-system}.


==> definitions/enterprise-system/lp.tex <==
enterprise systems%


==> definitions/enterprise-system/ls.tex <==
enterprise system%


==> definitions/enterprise-system/up.tex <==
Enterprise systems%


==> definitions/enterprise-system/us.tex <==
Enterprise system%


==> definitions/enterprise/def.tex <==
A work-system which performs a systematic and \emph{purposeful} activity.


==> definitions/enterprise/lp.tex <==
enterprises%


==> definitions/enterprise/ls.tex <==
enterprise%


==> definitions/enterprise/up.tex <==
Enterprises%


==> definitions/enterprise/us.tex <==
Enterprise%


==> definitions/environment-evolution/def.tex <==
The evolution of an \DN{environment} over time.


==> definitions/environment-evolution/lp.tex <==
environment evolutions%


==> definitions/environment-evolution/ls.tex <==
environment evolution%


==> definitions/environment-evolution/up.tex <==
Environment evolutions%


==> definitions/environment-evolution/us.tex <==
Environment evolution%


==> definitions/environment/def.tex <==
The environment of a \DN{domain} is that part of a \DN{viewer}'s \DN{conception} of a \DN{universe}, which has a direct \DN{link} to the \DN{domain}.



==> definitions/environment/lp.tex <==
environments%


==> definitions/environment/ls.tex <==
environment%


==> definitions/environment/up.tex <==
Environments%


==> definitions/environment/us.tex <==
Environment%


==> definitions/evolutionary-approach/def.tex <==
A (part of a) development process is executed completely in several iterations,
leading to several consecutive versions of the set of deliverables.


==> definitions/evolutionary-approach/lp.tex <==
evolutionary approaches%


==> definitions/evolutionary-approach/ls.tex <==
evolutionary approach%


==> definitions/evolutionary-approach/up.tex <==
Evolutionary approaches%


==> definitions/evolutionary-approach/us.tex <==
Evolutionary approach%


==> definitions/fact-oriented/def.tex <==
The fact-oriented \DefinitionName{approach}{ls} interprets sentences as 
facts about the \DefinitionName{uod}{ls}. This 
\DefinitionName{approach}{ls} is used data-intensive 
\DefinitionName{domain}{lp} when the structure of the 
\DefinitionName{data}{ls} is dominant. See also 
\DefinitionName{action-oriented}{ls}.


==> definitions/fact-oriented/lp.tex <==
fact oriented%


==> definitions/fact-oriented/ls.tex <==
fact oriented%


==> definitions/fact-oriented/up.tex <==
Fact oriented%


==> definitions/fact-oriented/us.tex <==
Fact oriented%


==> definitions/falsification/def.tex <==
A \DefinitionName{model}{ls} is assumed to be valid until contradicted 
by observation.


==> definitions/falsification/lp.tex <==
falsifications%


==> definitions/falsification/ls.tex <==
falsification%


==> definitions/falsification/up.tex <==
Falsifications%


==> definitions/falsification/us.tex <==
Falsification%


==> definitions/formal-communication/def.tex <==
\DefinitionName{communication}{us} that is based on an objective 
intermediate \DefinitionName{representation}{ls}, in which the 
\DefinitionName{information}{ls} transfer is independent of the actual 
interaction.


==> definitions/formal-communication/lp.tex <==
formal communications%


==> definitions/formal-communication/ls.tex <==
formal communication%


==> definitions/formal-communication/up.tex <==
Formal communications%


==> definitions/formal-communication/us.tex <==
Formal communication%


==> definitions/functional-requirement/def.tex <==
A \DN{requirement} which is based on the \DN{functionality} \DN{quality-attribute}.
 


==> definitions/functional-requirement/lp.tex <==
functional requirements%


==> definitions/functional-requirement/ls.tex <==
functional requirement%


==> definitions/functional-requirement/up.tex <==
Functional requirements%


==> definitions/functional-requirement/us.tex <==
Functional requirement%


==> definitions/functionality/lp.tex <==
functionalities%


==> definitions/functionality/ls.tex <==
functionality%


==> definitions/functionality/up.tex <==
Functionalities%


==> definitions/functionality/us.tex <==
Functionality%


==> definitions/goal-seeking-process/def.tex <==
A process seeking a balance between what \emph{ought to be} the case 
and what \emph{can be} the case with respect to some pre-existing 
situation, taking into acount the context, resource limitations, etc. 
Achieving the balance is the \DefinitionName{goal}{ls} sought after.


==> definitions/goal-seeking-process/lp.tex <==
goal-seeking processes%


==> definitions/goal-seeking-process/ls.tex <==
goal-seeking process%


==> definitions/goal-seeking-process/up.tex <==
Goal-seeking processes%


==> definitions/goal-seeking-process/us.tex <==
Goal-seeking process%


==> definitions/goal/def.tex <==
\AbbreviationOf{stakeholder-goal}


==> definitions/goal/lp.tex <==
goals%


==> definitions/goal/ls.tex <==
goal%


==> definitions/goal/up.tex <==
Goals%


==> definitions/goal/us.tex <==
Goal%


==> definitions/human-actor/def.tex <==
An \DN{actor} which is a single human being, or essentially a set of
human-beings, such as a team.



==> definitions/human-actor/lp.tex <==
human actors%


==> definitions/human-actor/ls.tex <==
human actor%


==> definitions/human-actor/up.tex <==
Human actors%


==> definitions/human-actor/us.tex <==
Human actors%


==> definitions/incremental-approach/def.tex <==
A (part of a) development process is executed on a sub-system by sub-system
basis, using some well-defined division of a system into sub-systems.


==> definitions/incremental-approach/lp.tex <==
incremental approaches%


==> definitions/incremental-approach/ls.tex <==
incremental approach%


==> definitions/incremental-approach/up.tex <==
Incremental approaches%


==> definitions/incremental-approach/us.tex <==
Incremental approach%


==> definitions/index-expression/def.tex <==
A simple structure for sentences, having some similarity with 
mathematical expressions. These expressions are used in the context of 
\DefinitionName{information}{us} Retrieval, as they provide a fair 
compromise between expressivity and feasibility. In the context of 
\DefinitionName{domain-modeling}{ls} they are a 
\DefinitionName{representation}{ls} for sentences structures in the 
contex of \DefinitionName{orm}{ls}.


==> definitions/index-expression/lp.tex <==
index expressions%


==> definitions/index-expression/ls.tex <==
index expression%


==> definitions/index-expression/up.tex <==
Index expressions%


==> definitions/index-expression/us.tex <==
Index expression%


==> definitions/informal-communication/def.tex <==
\DefinitionName{communication}{us} that is not based on an objective 
intermediate \DefinitionName{representation}{ls}, making the 
\DefinitionName{information}{ls} transfer independent of the actual 
interaction.


==> definitions/informal-communication/lp.tex <==
informal communications%


==> definitions/informal-communication/ls.tex <==
informal communication%


==> definitions/informal-communication/up.tex <==
Informal communications%


==> definitions/informal-communication/us.tex <==
Informal communication%


==> definitions/informant/def.tex <==
\Synonym{domain-expert}


==> definitions/informant/lp.tex <==
informants%


==> definitions/informant/ls.tex <==
informant%


==> definitions/informant/up.tex <==
Informants%


==> definitions/informant/us.tex <==
Informant%


==> definitions/information-architecture/def.tex <==
The \DN{architecture} of an \DN{information-system}.

Note that an information system may range in scope from, e.g., a value-chain wide 
information system to a hand-held information-appliance.


==> definitions/information-architecture/lp.tex <==
information architectures%


==> definitions/information-architecture/ls.tex <==
information architecture%


==> definitions/information-architecture/up.tex <==
Information architectures%


==> definitions/information-architecture/us.tex <==
Information architecture%


==> definitions/information-base/def.tex <==
The set of facts stored in an \DefinitionName{information-system}{ls}. 
This set contains all base statements that are valid in the associated 
\DefinitionName{uod}{ls}. If the 
\DefinitionName{closed-world-assumption}{ls} holds, then all other base 
statements are deemed to be false.


==> definitions/information-base/lp.tex <==
information bases%


==> definitions/information-base/ls.tex <==
information base%


==> definitions/information-base/up.tex <==
Information bases%


==> definitions/information-base/us.tex <==
Information base%


==> definitions/information-grammar/def.tex <==
A \DefinitionName{model}{ls} of the underlying format of the 
\DefinitionName{message}{lp} and to grasp the essentials of their 
meaning. This \DefinitionName{model}{ls} is seen as grammar.


==> definitions/information-grammar/lp.tex <==
information grammars%


==> definitions/information-grammar/ls.tex <==
information grammar%


==> definitions/information-grammar/up.tex <==
Information grammars%


==> definitions/information-grammar/us.tex <==
Information grammar%


==> definitions/information-intensive-organization/def.tex <==
An \DefinitionName{organization}{ls} conceived of as an 
\DefinitionName{organizational-system}{ls}, where the 
\DefinitionName{information-system}{ls} \DefinitionName{sub-system}{ls} 
forms an essential part of the 
\DefinitionName{organizational-system}{ls}.


==> definitions/information-intensive-organization/lp.tex <==
information intensive organizations%


==> definitions/information-intensive-organization/ls.tex <==
information intensive organization%


==> definitions/information-intensive-organization/up.tex <==
Information intensive organizations%


==> definitions/information-intensive-organization/us.tex <==
Information intensive organization%


==> definitions/information-processor/def.tex <==
The active \DefinitionName{component}{ls} of an 
\DefinitionName{information-system}{ls}. It processes the incoming 
commands.


==> definitions/information-processor/lp.tex <==
information processors%


==> definitions/information-processor/ls.tex <==
information processor%


==> definitions/information-processor/up.tex <==
Information processors%


==> definitions/information-processor/us.tex <==
Information processor%


==> definitions/information-system-engineering/def.tex <==
A system engineering process pertaining to the creation or change of \PDN{information-system}.


==> definitions/information-system-engineering/lp.tex <==
information system engineering%


==> definitions/information-system-engineering/ls.tex <==
information system engineering%


==> definitions/information-system-engineering/up.tex <==
Information system engineering%


==> definitions/information-system-engineering/us.tex <==
Information system engineering%


==> definitions/information-system/lp.tex <==
information systems%


==> definitions/information-system/ls.tex <==
information system%


==> definitions/information-system/up.tex <==
Information systems%


==> definitions/information-system/us.tex <==
Information system%


==> definitions/information-technology/def.tex <==
To be defined.


==> definitions/information-technology/lp.tex <==
information technologys%


==> definitions/information-technology/ls.tex <==
information technology%


==> definitions/information-technology/up.tex <==
Information technologys%


==> definitions/information-technology/us.tex <==
Information technology%


==> definitions/information/def.tex <==
The \DN{knowledge} increment brought about when a \DN{human-actor}
receives a message.  In other words, it is the difference between the
\PDN{conception} held by a \DN{human-actor} \emph{after} interpreting a
received \DN{message} and the \PDN{conception} held beforehand.


==> definitions/information/lp.tex <==
information%


==> definitions/information/ls.tex <==
information%


==> definitions/information/up.tex <==
Information%


==> definitions/information/us.tex <==
Information%


==> definitions/installation-process/def.tex <==
A process aiming to make a \DN{system} operational, i.e.\ to implement the use of the system by its prospective users.


==> definitions/installation-process/lp.tex <==
installation processes%


==> definitions/installation-process/ls.tex <==
installation process%


==> definitions/installation-process/up.tex <==
Installation processes%


==> definitions/installation-process/us.tex <==
Installation process%


==> definitions/interest/def.tex <==
The specific reason(s) why a \DN{viewer} observes a \DN{domain}.

In the case of a \DN{system}, this this is usually a confluence of the
\PDN{systemic-property} of \DN{interest} to the \DN{system-viewer} and the
aspects of the \DN{system} that are considered relevant (by the
\DN{system-viewer} to these \PDN{systemic-property}).


==> definitions/interest/lp.tex <==
interests%


==> definitions/interest/ls.tex <==
interest%


==> definitions/interest/up.tex <==
Interests%


==> definitions/interest/us.tex <==
Interest%


==> definitions/knowledge/def.tex <==
A relatively stable, and usually mostly consistent, set of \PDN{conception}
posessed by a single (possibly composed) \DN{actor}.

In more popular terms: ``an actor's picture of the world''.


==> definitions/knowledge/lp.tex <==
knowledge%


==> definitions/knowledge/ls.tex <==
knowledge%


==> definitions/knowledge/up.tex <==
Knowledge%


==> definitions/knowledge/us.tex <==
Knowledge%


==> definitions/linear-approach/def.tex <==
Step by step execution of a (part of a) development process, where a
consecutive step is not executed until the preceding step is finished.


==> definitions/linear-approach/lp.tex <==
linear approaches%


==> definitions/linear-approach/ls.tex <==
linear approach%


==> definitions/linear-approach/up.tex <==
Linear approaches%


==> definitions/linear-approach/us.tex <==
Linear approach%


==> definitions/link/def.tex <==
Any \DN{element} from a \DN{conception} that relates two \PDN{concept}.


==> definitions/link/lp.tex <==
links%


==> definitions/link/ls.tex <==
link%


==> definitions/link/up.tex <==
Links%


==> definitions/link/us.tex <==
Link%


==> definitions/lisa-d/def.tex <==
Language for \DefinitionName{information}{us} Structure and Access 
\DefinitionName{description}{up}. \DefinitionName{lisa-d}{us} has also 
a symbolic interpretation. In George Bernard Shaw's 'Pygmalion', 
professor Higgins, a linguistics prof, transforms Eliza Doolittle into 
a lady, speaking her language very well, though a bit 'robotic'.


==> definitions/lisa-d/lp.tex <==
Lisa-D%


==> definitions/lisa-d/ls.tex <==
Lisa-D%


==> definitions/lisa-d/up.tex <==
Lisa-D%


==> definitions/lisa-d/us.tex <==
Lisa-D%


==> definitions/maintainability/lp.tex <==
maintainabilities%


==> definitions/maintainability/ls.tex <==
maintainability%


==> definitions/maintainability/up.tex <==
Maintainabilities%


==> definitions/maintainability/us.tex <==
Maintainability%


==> definitions/maintenance/def.tex <==
A \DN{system} which is operational in its usage context, does not remain
operational by itself. Both technical and non-technical elements of the
\DN{system} need active maintenance to keep the \DN{system} operational
as is.


==> definitions/maintenance/lp.tex <==
maintenance%


==> definitions/maintenance/ls.tex <==
maintenance%


==> definitions/maintenance/up.tex <==
Maintenance%


==> definitions/maintenance/us.tex <==
Maintenance%


==> definitions/message/def.tex <==
\UDN{data} that is transmitted from one \DN{actor} (the sender) to another
\DN{actor} (the receiver).

A message may actually be `routed' via several \PDN{actor} before reaching its
actual receiver.  For example, when \DN{human-actor} exchange messages, they
usually need to make use of some other \DN{actor} playing the role of a medium
(for example, vibrations in the air, or an e-mail system).


==> definitions/message/lp.tex <==
messages%


==> definitions/message/ls.tex <==
message%


==> definitions/message/up.tex <==
Messages%


==> definitions/message/us.tex <==
Message%


==> definitions/meta-model/def.tex <==
A \DN{conception} of a \DN{viewer}'s \DN{viewpoint} on
the world.


==> definitions/meta-model/lp.tex <==
meta models%


==> definitions/meta-model/ls.tex <==
meta model%


==> definitions/meta-model/up.tex <==
Meta models%


==> definitions/meta-model/us.tex <==
Meta model%


==> definitions/method-fragment/lp.tex <==
method fragments%


==> definitions/method-fragment/ls.tex <==
method fragment%


==> definitions/method-fragment/up.tex <==
Method fragments%


==> definitions/method-fragment/us.tex <==
Method fragment%


==> definitions/method/def.tex <==
An integrated combination of a: \DefinitionName{way-of-thinking}{ls}, \DefinitionName{way-of-controlling}{ls}, \DefinitionName{way-of-working}{ls}, \DefinitionName{way-of-modeling}{ls} (a 
\DefinitionName{technique}{ls}), and a \DefinitionName{way-of-supporting}{ls} aimed at obtaining 
results. 


==> definitions/method/lp.tex <==
methods%


==> definitions/method/ls.tex <==
method%


==> definitions/method/up.tex <==
Methods%


==> definitions/method/us.tex <==
Method%


==> definitions/model-builder/def.tex <==
The person involved in the formal dialog with the 
\DefinitionName{modeling-mediator}{ls}, processing the semi-formal 
specifications provided by the \DefinitionName{modeling-mediator}{ls}. 
The combination of \DefinitionName{modeling-mediator}{ls} and 
\DefinitionName{model-builder}{ls} is also referred to as 
\DefinitionName{system-analyst}{ls}.


==> definitions/model-builder/lp.tex <==
model builders%


==> definitions/model-builder/ls.tex <==
model builder%


==> definitions/model-builder/up.tex <==
Model builders%


==> definitions/model-builder/us.tex <==
Model builder%


==> definitions/model-concept/def.tex <==
A \DN{concept} from a \DN{conception} which is a \DN{model}. 


==> definitions/model-concept/lp.tex <==
model concepts%


==> definitions/model-concept/ls.tex <==
model concept%


==> definitions/model-concept/up.tex <==
Model concepts%


==> definitions/model-concept/us.tex <==
Model concept%


==> definitions/model-element/def.tex <==
An \DN{element} from a \DN{conception} which is a \DN{model}. 


==> definitions/model-element/lp.tex <==
model elements%


==> definitions/model-element/ls.tex <==
model element%


==> definitions/model-element/up.tex <==
Model elements%


==> definitions/model-element/us.tex <==
Model element%


==> definitions/model-link/def.tex <==
A \DN{link} from a \DN{conception} which is a \DN{model}. 


==> definitions/model-link/lp.tex <==
model links%


==> definitions/model-link/ls.tex <==
model link%


==> definitions/model-link/up.tex <==
Model links%


==> definitions/model-link/us.tex <==
Model link%


==> definitions/model-relation-type/lp.tex <==
model relation types%


==> definitions/model-relation-type/ls.tex <==
model relation type%


==> definitions/model-relation-type/up.tex <==
Model relation types%


==> definitions/model-relation-type/us.tex <==
Model relation type%


==> definitions/model/def.tex <==
A purposely abstracted \DN{domain} (possibly in conjunction with its \DN{environment})
of some `part' or `aspect' of the \DN{universe} a \DN{viewer} may have an \DN{interest}
in.

For practical reasons, a \DN{model} will typically be consistent and
unambiguous with regards to some underlying semantic domain, such as logic.


==> definitions/model/lp.tex <==
models%


==> definitions/model/ls.tex <==
model%


==> definitions/model/up.tex <==
Models%


==> definitions/model/us.tex <==
Model%


==> definitions/modeling-fragment/lp.tex <==
modeling fragments%


==> definitions/modeling-fragment/ls.tex <==
modeling fragment%


==> definitions/modeling-fragment/up.tex <==
Modeling fragments%


==> definitions/modeling-fragment/us.tex <==
Modeling fragment%


==> definitions/modeling-mediator/def.tex <==
The person involved in the informal dialog with the 
\DefinitionName{domain-expert}{ls}, mediating between the 
\DefinitionName{domain-expert}{ls} and the 
\DefinitionName{model-builder}{ls}. The combination of 
\DefinitionName{modeling-mediator}{ls} and 
\DefinitionName{model-builder}{ls} is also referred to as 
\DefinitionName{system-analyst}{ls}.


==> definitions/modeling-mediator/lp.tex <==
modeling mediators%


==> definitions/modeling-mediator/ls.tex <==
modeling mediator%


==> definitions/modeling-mediator/up.tex <==
Modeling mediators%


==> definitions/modeling-mediator/us.tex <==
Modeling mediator%


==> definitions/modeling-technique/def.tex <==
The combination of a \DN{way-of-modeling} and a \DN{way-of-communicating}.



==> definitions/modeling-technique/lp.tex <==
modeling techniques%


==> definitions/modeling-technique/ls.tex <==
modeling technique%


==> definitions/modeling-technique/up.tex <==
Modeling techniques%


==> definitions/modeling-technique/us.tex <==
Modeling technique%


==> definitions/modeling/def.tex <==
The act of purposely abstracting a \DN{model} from (what is conceived to be) a part
of the \DN{universe}.



==> definitions/modeling/lp.tex <==
modeling%


==> definitions/modeling/ls.tex <==
modeling%


==> definitions/modeling/up.tex <==
Modeling%


==> definitions/modeling/us.tex <==
Modeling%


==> definitions/new <==
#!/bin/bash
echo -n "lower case singular name: "
read LS

function Upper () {
  echo `echo $1 | sed -e "s/^./&##/" | sed -e "s/##.*//" | tr [:lower:] [:upper:]``echo $1 | sed -e "s/^.//"`
}

KEY="`echo $LS | sed -e "s/ /-/g"`"
LP="`echo "$LS"s \
     | sed -e "s/cys/cy/"    \
     | sed -e "s/ings$/ing/" \
     | sed -e "s/chs$/ches/" \
     | sed -e "s/sss$/sses/" \
     | sed -e "s/tys$/ties/" \
     | cat`"
US="`Upper "$LS"`"
UP="`Upper "$LP"`"

echo "key                     : [$KEY]"
echo "lower case singular name: [$LS]"
echo "lower case plural   name: [$LP]"
echo "upper case singular name: [$US]"
echo "upper case plural   name: [$UP]"

mkdir $KEY
echo $LS% > $KEY/ls.tex
echo $LP% > $KEY/lp.tex
echo $US% > $KEY/us.tex
echo $UP% > $KEY/up.tex
vi $KEY/def.tex


==> definitions/niam/def.tex <==
aN \DefinitionName{information}{us} Analysis \DefinitionName{method}{us}


==> definitions/niam/lp.tex <==
NIAM%


==> definitions/niam/ls.tex <==
NIAM%


==> definitions/niam/up.tex <==
NIAM%


==> definitions/niam/us.tex <==
NIAM%


==> definitions/non-functional-requirement/def.tex <==
A \DN{requirement} which is not a \DN{functional-requirement}.



==> definitions/non-functional-requirement/lp.tex <==
non-functional requirements%


==> definitions/non-functional-requirement/ls.tex <==
non-functional requirement%


==> definitions/non-functional-requirement/up.tex <==
Non-functional requirements%


==> definitions/non-functional-requirement/us.tex <==
Non-functional requirement%


==> definitions/ockhams-razor/def.tex <==
The simplest explanation is usually the best.


==> definitions/ockhams-razor/lp.tex <==
Ockham's Razor%


==> definitions/ockhams-razor/ls.tex <==
Ockham's Razor%


==> definitions/ockhams-razor/up.tex <==
Ockham's Razor%


==> definitions/ockhams-razor/us.tex <==
Ockham's Razor%


==> definitions/ontology/def.tex <==
The subject of \DefinitionName{ontology}{ls} is the study of the 
categories of things that exist or may exist in some 
\DefinitionName{domain}{ls}. The product of such a study, called an 
\DefinitionName{ontology}{ls}, is a catalog of the types of things that 
are assumed to exist in a \DefinitionName{domain}{ls} of 
\DefinitionName{interest}{ls} $D$ from the 
\DefinitionName{perspective}{ls} of a person who uses a language $L$ 
for the purpose of talking about $D$. The types in the 
\DefinitionName{ontology}{ls} represent the predicates, word senses, or 
\DefinitionName{concept}{ls} and relation types of the language $L$ 
when used to discuss topics in the \DefinitionName{domain}{ls} $D$.


==> definitions/ontology/lp.tex <==
ontologies%


==> definitions/ontology/ls.tex <==
ontology%


==> definitions/ontology/up.tex <==
Ontologies%


==> definitions/ontology/us.tex <==
Ontology%


==> definitions/open-active-system/def.tex <==
A \DN{system} that is an \DN{open-system} as well as an \DN{active-system}.


==> definitions/open-active-system/lp.tex <==
open active systems%


==> definitions/open-active-system/ls.tex <==
open active system%


==> definitions/open-active-system/up.tex <==
Open active systems%


==> definitions/open-active-system/us.tex <==
Open active system%


==> definitions/open-system/def.tex <==
A special kind of \DN{dynamic-system} that is conceived as reacting to external
triggers, i.e.\ there may be changes inside the system due to external causes
originating from the system's \DN{environment}.


==> definitions/open-system/lp.tex <==
open systems%


==> definitions/open-system/ls.tex <==
open system%


==> definitions/open-system/up.tex <==
Open systems%


==> definitions/open-system/us.tex <==
Open system%


==> definitions/organization/def.tex <==
A group of \PDN{actor} with a purpose, who:
\begin{itemize}
   \item interact with each other,
   \item form a network of roles,
   \item make use of (the services of) other actors.
\end{itemize}
An \DN{organization} in itself is an \DN{actor} as well, and may as such
participate in yet another \PDN{organization}.


==> definitions/organization/lp.tex <==
organizations%


==> definitions/organization/ls.tex <==
organization%


==> definitions/organization/up.tex <==
Organizations%


==> definitions/organization/us.tex <==
Organization%


==> definitions/organizational-system/lp.tex <==
organizational systems%


==> definitions/organizational-system/ls.tex <==
organizational system%


==> definitions/organizational-system/up.tex <==
Organizational systems%


==> definitions/organizational-system/us.tex <==
Organizational system%


==> definitions/orm/def.tex <==
Object-Role \DefinitionName{modeling}{us}


==> definitions/orm/lp.tex <==
ORM%


==> definitions/orm/ls.tex <==
ORM%


==> definitions/orm/up.tex <==
ORM%


==> definitions/orm/us.tex <==
ORM%


==> definitions/ornf/def.tex <==
Object Role Normalform, a \DefinitionName{controlled-language}{ls} 
developed in the context of object-role \DefinitionName{modeling}{ls}.


==> definitions/ornf/lp.tex <==
ORNF%


==> definitions/ornf/ls.tex <==
ORNF%


==> definitions/ornf/up.tex <==
ORNF%


==> definitions/ornf/us.tex <==
ORNF%


==> definitions/patiens/def.tex <==
The role in a sentence that most commonly is associated with the 
grammatical object.


==> definitions/patiens/lp.tex <==
patiens%


==> definitions/patiens/ls.tex <==
patiens%


==> definitions/patiens/up.tex <==
Patiens%


==> definitions/patiens/us.tex <==
Patiens%


==> definitions/perception/def.tex <==
That what results, in the mind of a \DN{viewer}, when they observe a
\DN{domain} with their senses, and forms a specific pattern of visual, auditory
or other sensations in their minds.


==> definitions/perception/lp.tex <==
perceptions%


==> definitions/perception/ls.tex <==
perception%


==> definitions/perception/up.tex <==
Perceptions%


==> definitions/perception/us.tex <==
Perception%


==> definitions/perspective/def.tex <==
A set of related \DN{interests} in terms of which \PDN{viewer} may observe a
\DN{domain}. 


==> definitions/perspective/lp.tex <==
perspectives%


==> definitions/perspective/ls.tex <==
perspective%


==> definitions/perspective/perspective/def.tex <==
A set of related \PDN{interest} in terms of which \PDN{viewer} may observe a
\DN{domain}. 


==> definitions/perspective/perspective/lp.tex <==
perspectives%


==> definitions/perspective/perspective/ls.tex <==
perspective%


==> definitions/perspective/perspective/up.tex <==
Perspectives%


==> definitions/perspective/perspective/us.tex <==
Perspective%


==> definitions/perspective/up.tex <==
Perspectives%


==> definitions/perspective/us.tex <==
Perspective%


==> definitions/portability/lp.tex <==
portabilities%


==> definitions/portability/ls.tex <==
portability%


==> definitions/portability/up.tex <==
Portabilities%


==> definitions/portability/us.tex <==
Portability%


==> definitions/process-requirement/def.tex <==
A \DN{requirement} pertaining to the actual \DN{system-engineering}
\emph{process}.


==> definitions/process-requirement/lp.tex <==
process requirements%


==> definitions/process-requirement/ls.tex <==
process requirement%


==> definitions/process-requirement/up.tex <==
Process requirements%


==> definitions/process-requirement/us.tex <==
Process requirement%


==> definitions/product-requirement/def.tex <==
A \DN{requirement} on any of the products, pertaining to a \DN{system} as it
will eventually result from a \DN{system-engineering} process.


==> definitions/product-requirement/lp.tex <==
product requirements%


==> definitions/product-requirement/ls.tex <==
product requirement%


==> definitions/product-requirement/up.tex <==
Product requirements%


==> definitions/product-requirement/us.tex <==
Product requirement%


==> definitions/psm/def.tex <==
Predicator Set \DefinitionName{model}{us}


==> definitions/psm/lp.tex <==
PSM%


==> definitions/psm/ls.tex <==
PSM%


==> definitions/psm/up.tex <==
PSM%


==> definitions/psm/us.tex <==
PSM%


==> definitions/quality-attribute/def.tex <==
A specific class of \PDN{quality-property}.


==> definitions/quality-attribute/lp.tex <==
quality attributes%


==> definitions/quality-attribute/ls.tex <==
quality attribute%


==> definitions/quality-attribute/up.tex <==
Quality attributes%


==> definitions/quality-attribute/us.tex <==
Quality attribute%


==> definitions/quality-property/def.tex <==
A \DN{systemic-property}, used to describe and asses the \DN{quality} of a \DN{system}.


==> definitions/quality-property/lp.tex <==
quality properties%


==> definitions/quality-property/ls.tex <==
quality property%


==> definitions/quality-property/up.tex <==
Quality properties%


==> definitions/quality-property/us.tex <==
Quality property%


==> definitions/quality/def.tex <==
Is the totality of \PDN{systemic-property} of a \DN{system} that relate
to its ability to satisfy stated and/or implied needs.


==> definitions/quality/lp.tex <==
qualities%


==> definitions/quality/ls.tex <==
quality%


==> definitions/quality/up.tex <==
Qualities%


==> definitions/quality/us.tex <==
Quality%


==> definitions/reactive-system/def.tex <==
An \DN{open-active-system} where each expression of the system is a reaction,
and where each impression immediately causes a reaction.



==> definitions/reactive-system/lp.tex <==
reactive systems%


==> definitions/reactive-system/ls.tex <==
reactive system%


==> definitions/reactive-system/up.tex <==
Reactive systems%


==> definitions/reactive-system/us.tex <==
Reactive system%


==> definitions/realization-process/def.tex <==
The combination of a \DefinitionName{construction-process}{ls} and a 
\DefinitionName{deployment-process}{ls}. \Where{construction-process} 
\Where{deployment-process}


==> definitions/realization-process/lp.tex <==
realization processes%


==> definitions/realization-process/ls.tex <==
realization process%


==> definitions/realization-process/up.tex <==
Realization processes%


==> definitions/realization-process/us.tex <==
Realization process%


==> definitions/reliability/lp.tex <==
reliabilities%


==> definitions/reliability/ls.tex <==
reliability%


==> definitions/reliability/up.tex <==
Reliabilities%


==> definitions/reliability/us.tex <==
Reliability%


==> definitions/representation/def.tex <==
The result of a \DN{viewer} denoting a \DN{conception}, using
some language and medium to express themselves.



==> definitions/representation/lp.tex <==
representations%


==> definitions/representation/ls.tex <==
representation%


==> definitions/representation/up.tex <==
Representations%


==> definitions/representation/us.tex <==
Representation%


==> definitions/requirement/def.tex <==
an essential \DN{quality-property} that a \DN{system} or its \DN{system-description} has to satisfy.



==> definitions/requirement/lp.tex <==
requirements%


==> definitions/requirement/ls.tex <==
requirement%


==> definitions/requirement/up.tex <==
Requirements%


==> definitions/requirement/us.tex <==
Requirement%


==> definitions/responsive-system/def.tex <==
An \DN{open-active-system} (possibly also a \DN{reactive-system}) where it holds
for at least one expression that a certain impression or a temporal pattern of
impressions is a necessary, but not a sufficient dynamic condition for its
occurrence.  The receipt of an order is a necessary impression to a ``sales
system'', for the expression ``delivery of the ordered goods", but it is not a
sufficient condition.



==> definitions/responsive-system/lp.tex <==
responsive systems%


==> definitions/responsive-system/ls.tex <==
responsive system%


==> definitions/responsive-system/up.tex <==
Responsive systems%


==> definitions/responsive-system/us.tex <==
Responsive system%


==> definitions/ridl/def.tex <==
Reference and IDea Language


==> definitions/ridl/lp.tex <==
RIDL%


==> definitions/ridl/ls.tex <==
RIDL%


==> definitions/ridl/up.tex <==
RIDL%


==> definitions/ridl/us.tex <==
RIDL%


==> definitions/run-time-requirement/def.tex <==
A \DN{product-requirement} on a \DN{system} as it will eventually result from a
\DN{system-engineering} process.

These requirements usually refer to \PDN{quality-attribute} such as:
\DN{functionality}, \DN{usability}, \DN{efficiency} and \DN{reliability}.

Note that these requirements are observable as \PDN{systemic-property} of the
system resulting from the development process.


==> definitions/run-time-requirement/lp.tex <==
run-time requirements%


==> definitions/run-time-requirement/ls.tex <==
run-time requirement%


==> definitions/run-time-requirement/up.tex <==
Run-time requirements%


==> definitions/run-time-requirement/us.tex <==
Run-time requirement%


==> definitions/shadow-world/def.tex <==
A (usually formal) world that keeps track of the wheeling and reeling 
in the \DefinitionName{uod}{ls}.


==> definitions/shadow-world/lp.tex <==
shadow worlds%


==> definitions/shadow-world/ls.tex <==
shadow world%


==> definitions/shadow-world/up.tex <==
Shadow worlds%


==> definitions/shadow-world/us.tex <==
Shadow world%


==> definitions/simulation/def.tex <==
The imitative \DefinitionName{representation}{ls} of the functioning of 
one \DefinitionName{system}{ls} by means of the functioning of another.


==> definitions/simulation/lp.tex <==
simulations%


==> definitions/simulation/ls.tex <==
simulation%


==> definitions/simulation/up.tex <==
Simulations%


==> definitions/simulation/us.tex <==
Simulation%


==> definitions/sql/def.tex <==
Structured Query Language


==> definitions/sql/lp.tex <==
SQL%


==> definitions/sql/ls.tex <==
SQL%


==> definitions/sql/up.tex <==
SQL%


==> definitions/sql/us.tex <==
SQL%


==> definitions/stakeholder-concern/def.tex <==
An \DN{interest} of a \DN{stakeholder}, resulting from the stakeholder's
\DN{goal}, and the role played by some \DN{system}.

This usually pertains to the system's engineering, its operation or any other
aspects that are critical or otherwise important to one or more stakeholders. 


==> definitions/stakeholder-concern/lp.tex <==
stakeholder concerns%


==> definitions/stakeholder-concern/ls.tex <==
stakeholder concern%


==> definitions/stakeholder-concern/up.tex <==
Stakeholder concerns%


==> definitions/stakeholder-concern/us.tex <==
Stakeholder concern%


==> definitions/stakeholder-goal/def.tex <==
The end toward which effort is directed by a \DN{stakeholder}, in which the
\DN{system} (of which the stakeholder is indeed a stakeholder) plays a role.

This may pertain to strategic, tactical or operational end.  The role of the
system may range from passive to active. For example, a financial controller's
goal with regards to a future/changed system may be to control engineering
costs, while the goal of users of the system may be to get their job done more
efficiently.


==> definitions/stakeholder-goal/lp.tex <==
stakeholder goals%


==> definitions/stakeholder-goal/ls.tex <==
stakeholder goal%


==> definitions/stakeholder-goal/up.tex <==
Stakeholder goals%


==> definitions/stakeholder-goal/us.tex <==
Stakeholder goal%


==> definitions/stakeholder-requirement/def.tex <==
A \DN{requirement} posed on a future/changed \DN{system} by a
specific \DN{stakeholder}.

These requirements should essentially be refinements of the 
\PDN{stakeholder-concern}.


==> definitions/stakeholder-requirement/lp.tex <==
stakeholder requirements%


==> definitions/stakeholder-requirement/ls.tex <==
stakeholder requirement%


==> definitions/stakeholder-requirement/up.tex <==
Stakeholder requirements%


==> definitions/stakeholder-requirement/us.tex <==
Stakeholder requirement%


==> definitions/stakeholder-requirements-description/def.tex <==
A \DN{system-description} of the \PDN{stakeholder-requirement} on a
future/changed \DN{system} $S$, which covers:
\begin{itemize}
   \item the \PDN{requirement} which will be imposed by the \DN{environment} on
   system $S$ and
   \item the \PDN{requirement} on other systems in the environment of system
   $S$ which system $S$ may/must use for its own purposes.

   For example: the properties of a given infrastructure that must/may be used, 
   `legacy' systems with which $S$ needs to interface, etc.
\end{itemize}
The gap between these sets of \PDN{requirement}, is what needs to be `designed
in' by the \DN{design-process}.



==> definitions/stakeholder-requirements-description/lp.tex <==
stakeholder requirements descriptions%


==> definitions/stakeholder-requirements-description/ls.tex <==
stakeholder requirements description%


==> definitions/stakeholder-requirements-description/up.tex <==
Stakeholder requirements descriptions%


==> definitions/stakeholder-requirements-description/us.tex <==
Stakeholder requirements description%


==> definitions/stakeholder/def.tex <==
Some actor in a \DN{system-engineering-community} with a specific stake
pertaining to a system's development, its operation or any other aspects that
are critical or otherwise important.

Examples are: Users, operators, owners, architects, engineers, testers,
project managers, business management, ...



==> definitions/stakeholder/lp.tex <==
stakeholders%


==> definitions/stakeholder/ls.tex <==
stakeholder%


==> definitions/stakeholder/up.tex <==
Stakeholders%


==> definitions/stakeholder/us.tex <==
Stakeholder%


==> definitions/standard-name/def.tex <==
An agreed standard denotation for objects and things.


==> definitions/standard-name/lp.tex <==
standard names%


==> definitions/standard-name/ls.tex <==
standard name%


==> definitions/standard-name/up.tex <==
Standard names%


==> definitions/standard-name/us.tex <==
Standard names%


==> definitions/strong-identification/def.tex <==
A sufficient condition to be able to uniquely identify objects and 
things, stating each object has a \DefinitionName{standard-name}{ls} 
derived from the associated object type.


==> definitions/strong-identification/lp.tex <==
strong identification%


==> definitions/strong-identification/ls.tex <==
strong identification%


==> definitions/strong-identification/up.tex <==
Strong identification%


==> definitions/strong-identification/us.tex <==
Strong identification%


==> definitions/sub-system/def.tex <==
A sub-system $S'$ of a \DN{system} $S$, is a \DN{system} where the set of
\PDN{element} in $S'$ is a subset of the \PDN{element} in $S$.


==> definitions/sub-system/lp.tex <==
sub-systems%


==> definitions/sub-system/ls.tex <==
sub-system%


==> definitions/sub-system/up.tex <==
Sub-systems%


==> definitions/sub-system/us.tex <==
Sub-system%


==> definitions/system-activity/def.tex <==
A \DN{system-concept} that is conceived of as changing parts of the
\DN{universe}.


==> definitions/system-activity/lp.tex <==
system activities%


==> definitions/system-activity/ls.tex <==
system activity%


==> definitions/system-activity/up.tex <==
System activities%


==> definitions/system-activity/us.tex <==
System activity%


==> definitions/system-analyst/def.tex <==
A person constructing a \DefinitionName{model}{ls} of a 
\DefinitionName{uod}{ls} from a semi-formal specification. Also 
referred as \DefinitionName{model-builder}{ls}.


==> definitions/system-analyst/lp.tex <==
system analysts%


==> definitions/system-analyst/ls.tex <==
system analyst%


==> definitions/system-analyst/up.tex <==
System analysts%


==> definitions/system-analyst/us.tex <==
System analyst%


==> definitions/system-builder/def.tex <==
A person constructing a \DefinitionName{model}{ls} of a 
\DefinitionName{uod}{ls} from a semi-formal specification. Also 
referred to as \DefinitionName{system-analyst}{ls}.


==> definitions/system-builder/lp.tex <==
system builders%


==> definitions/system-builder/ls.tex <==
system builder%


==> definitions/system-builder/up.tex <==
System builder%


==> definitions/system-builder/us.tex <==
System builder%


==> definitions/system-concept/def.tex <==
Any element from a \DN{system} that is a \DN{concept}.


==> definitions/system-concept/lp.tex <==
system concepts%


==> definitions/system-concept/ls.tex <==
system concept%


==> definitions/system-concept/up.tex <==
System concepts%


==> definitions/system-concept/us.tex <==
System concept%


==> definitions/system-description/def.tex <==
The \DN{description} of a \DN{system}.


==> definitions/system-description/lp.tex <==
system descriptions%


==> definitions/system-description/up.tex <==
System descriptions%


==> definitions/system-description/us.tex <==
System description%


==> definitions/system-design/def.tex <==
To do


==> definitions/system-design/lp.tex <==
system designs%


==> definitions/system-design/ls.tex <==
system design%


==> definitions/system-design/up.tex <==
System designs%


==> definitions/system-design/us.tex <==
System design%


==> definitions/system-development-community/def.tex <==
A group of objects, such as actors and representations, which are involved in
the development of a system.


==> definitions/system-development-community/lp.tex <==
system development communities%


==> definitions/system-development-community/ls.tex <==
system development community%


==> definitions/system-development-community/up.tex <==
System development communities%


==> definitions/system-development-community/us.tex <==
System development community%


==> definitions/system-development/def.tex <==
To be done


==> definitions/system-development/lp.tex <==
system developments%


==> definitions/system-development/ls.tex <==
system development%


==> definitions/system-development/up.tex <==
System developments%


==> definitions/system-development/us.tex <==
System development%


==> definitions/system-domain/def.tex <==
A \DN{domain} that is conceived to be a \DN{system}, by some \DN{viewer}, by
the distinction from its \DN{environment}, by its coherence, and because of its
\DN{systemic-property}.


==> definitions/system-domain/lp.tex <==
system domains%


==> definitions/system-domain/ls.tex <==
system domain%


==> definitions/system-domain/up.tex <==
System domains%


==> definitions/system-domain/us.tex <==
System domain%


==> definitions/system-element/def.tex <==
Any element from a \DN{system}.


==> definitions/system-element/lp.tex <==
system elements%


==> definitions/system-element/ls.tex <==
system element%


==> definitions/system-element/up.tex <==
System elements%


==> definitions/system-element/us.tex <==
System element%


==> definitions/system-engineering-community/def.tex <==
A group of objects, such as actors and representations, which are involved in
a system engineering process.


==> definitions/system-engineering-community/lp.tex <==
system engineering communities%


==> definitions/system-engineering-community/ls.tex <==
system engineering community%


==> definitions/system-engineering-community/up.tex <==
System engineering communities%


==> definitions/system-engineering-community/us.tex <==
System engineering community%


==> definitions/system-engineering/def.tex <==
A process involving aimed at producing a changed system, involving the
execution of four sub-processes: \DO{definition-process}{definition},
\DO{design-process}{design}, \DO{construction-process}{construction} and
\DO{installation-process}{installation} of the \DN{system}.  Processes that
may be executed sequentially, incrementally, interleaved, or in parallel.


==> definitions/system-engineering/lp.tex <==
system engineering%


==> definitions/system-engineering/ls.tex <==
system engineering%


==> definitions/system-engineering/up.tex <==
System engineering%


==> definitions/system-engineering/us.tex <==
System engineering%


==> definitions/system-evolution/def.tex <==
The evolution, over time, of a system. 


==> definitions/system-evolution/lp.tex <==
system evolutions%


==> definitions/system-evolution/ls.tex <==
system evolution%


==> definitions/system-evolution/up.tex <==
System evolutions%


==> definitions/system-evolution/us.tex <==
System evolution%


==> definitions/system-exposition/lp.tex <==
system expositions%


==> definitions/system-exposition/ls.tex <==
system exposition%


==> definitions/system-exposition/up.tex <==
System expositions%


==> definitions/system-exposition/us.tex <==
System exposition%


==> definitions/system-link/def.tex <==
Any element from a \DN{system} that is a \DN{link}.


==> definitions/system-link/lp.tex <==
system links%


==> definitions/system-link/ls.tex <==
system link%


==> definitions/system-link/up.tex <==
System links%


==> definitions/system-link/us.tex <==
System link%


==> definitions/system-mission/def.tex <==
A role, to the benefit of \PDN{stakeholder-goal}, for which the
\DN{system} is intended.


==> definitions/system-mission/lp.tex <==
system missions%


==> definitions/system-mission/ls.tex <==
system mission%


==> definitions/system-mission/up.tex <==
System missions%


==> definitions/system-mission/us.tex <==
System mission%


==> definitions/system-model/def.tex <==
A \DN{model} of a \DN{system}.


==> definitions/system-model/lp.tex <==
system models%


==> definitions/system-model/ls.tex <==
system model%


==> definitions/system-model/up.tex <==
System models%


==> definitions/system-model/us.tex <==
System model%


==> definitions/system-requirement/def.tex <==
A \DN{requirement} on a future/changed \DN{system}.  These requirements are
usually an negotiated integration of \PDN{stakeholder-requirement} and should
essentially be refinements of the \DN{system-mission}.


==> definitions/system-requirement/lp.tex <==
system requirements%


==> definitions/system-requirement/ls.tex <==
system requirement%


==> definitions/system-requirement/up.tex <==
System requirements%


==> definitions/system-requirement/us.tex <==
System requirement%


==> definitions/system-requirements-description/def.tex <==
A \DN{system-description} of the \PDN{system-requirement} on a future/changed
\DN{system} $S$, which covers:
\begin{itemize}
   \item the \PDN{requirement} which will be imposed by the \DN{environment} on
   system $S$ and
   \item the \PDN{requirement} on other systems in the environment of system
   $S$ which system $S$ may/must use for its own purposes.

   For example: the properties of a given infrastructure that must/may be used,
   `legacy' systems with which $S$ needs to interface, etc.
\end{itemize}
The gap between these sets of requirements, is what needs to be `designed in'
by the \DN{design-process}.



==> definitions/system-requirements-description/lp.tex <==
system requirements descriptions%


==> definitions/system-requirements-description/ls.tex <==
system requirements description%


==> definitions/system-requirements-description/up.tex <==
System requirements descriptions%


==> definitions/system-requirements-description/us.tex <==
System requirements description%


==> definitions/system-type/def.tex <==
A type that determines the potential kinds of \PDN{systemic-property},
\PDN{element} of the \DN{system-domain} and roles of the \PDN{element} in
achieving the \PDN{systemic-property}.



==> definitions/system-type/lp.tex <==
system types%


==> definitions/system-type/ls.tex <==
system type%


==> definitions/system-type/up.tex <==
System types%


==> definitions/system-type/us.tex <==
System type%


==> definitions/system-view/def.tex <==
A \DN{model} of a \DN{system-domain} from the perspective of a related set of 
\PDN{interest} of a \DN{system-viewer}.


==> definitions/system-view/lp.tex <==
system views%


==> definitions/system-view/ls.tex <==
system view%


==> definitions/system-view/up.tex <==
System views%


==> definitions/system-view/us.tex <==
System view%


==> definitions/system-viewer/def.tex <==
A \DN{viewer} of a \DN{system-domain}.



==> definitions/system-viewer/lp.tex <==
system viewers%


==> definitions/system-viewer/ls.tex <==
system viewer%


==> definitions/system-viewer/up.tex <==
System viewers%


==> definitions/system-viewer/us.tex <==
System viewer%


==> definitions/system-viewpoint/def.tex <==
A specification of the conventions for constructing and using \PDN{system-view}.

This involves:
  a \DN{way-of-thinking}, 
  a \DN{way-of-modeling}, 
  a \DN{way-of-communicating},
  a \DN{way-of-working},
  a \DN{way-of-supporting} and
  a \DN{way-of-using}



==> definitions/system-viewpoint/lp.tex <==
system viewpoints%


==> definitions/system-viewpoint/ls.tex <==
system viewpoint%


==> definitions/system-viewpoint/up.tex <==
System viewpoints%


==> definitions/system-viewpoint/us.tex <==
System viewpoint%


==> definitions/system/def.tex <==
A special \DN{model} of a \DN{system-domain}, whereby all the things contained
in that model are transitively coherent, i.e.\ all of them are directly or
indirectly related to each other and form a coherent whole.

A system is conceived as having assigned to it, as a whole, a specific
characterization (a non-empty set of \PDN{systemic-property}) which, in
general, cannot be attributed exclusively to any of its components.


==> definitions/system/lp.tex <==
systems%


==> definitions/system/ls.tex <==
system%


==> definitions/system/up.tex <==
Systems%


==> definitions/system/us.tex <==
System%


==> definitions/systemic-property/def.tex <==
A meaningful relationship that exists between the \DN{domain} of elements
considered as a whole, the \DN{system-domain} and its \DN{environment}.


==> definitions/systemic-property/lp.tex <==
systemic properties%


==> definitions/systemic-property/ls.tex <==
systemic property%


==> definitions/systemic-property/up.tex <==
Systemic properties%


==> definitions/systemic-property/us.tex <==
Systemic property%


==> definitions/technique-relation/def.tex <==
A well-defined relation between the sets of \DefinitionName{model}{lp} 
that may be represented in a \DefinitionName{technique}{ls}. An example 
would be a mapping algorithm between a conceptual \DefinitionName{model}{ls} and 
a relational database schema, the relation between the \DefinitionName{concept}{lp} of a business 
process \DefinitionName{model}{ls} and the concepts of a supporting work-flow, etc.


==> definitions/technique-relation/lp.tex <==
technique relations%


==> definitions/technique-relation/ls.tex <==
technique relation%


==> definitions/technique-relation/up.tex <==
Technique relations%


==> definitions/technique-relation/us.tex <==
Technique relation%


==> definitions/technique/def.tex <==
\Synonym{way-of-modeling}


==> definitions/technique/lp.tex <==
techniques%


==> definitions/technique/ls.tex <==
technique%


==> definitions/technique/up.tex <==
Techniques%


==> definitions/technique/us.tex <==
Technique%


==> definitions/telephone-heuristic/def.tex <==
\DefinitionName{communication}{us} form where the way to carry over 
\DefinitionName{information}{ls} is by written text.


==> definitions/telephone-heuristic/lp.tex <==
telephone heuristics%


==> definitions/telephone-heuristic/ls.tex <==
telephone heuristic%


==> definitions/telephone-heuristic/up.tex <==
Telephone heuristics%


==> definitions/telephone-heuristic/us.tex <==
Telephone heuristic%


==> definitions/turing-test/def.tex <==
An test to see if an human can make the distinction between the program 
in question and a human respondent.


==> definitions/turing-test/lp.tex <==
Turing tests%


==> definitions/turing-test/ls.tex <==
Turing test%


==> definitions/turing-test/up.tex <==
Turing tests%


==> definitions/turing-test/us.tex <==
Turing test%


==> definitions/uml/def.tex <==
Unified \DefinitionName{modeling}{us} Language


==> definitions/uml/lp.tex <==
UML%


==> definitions/uml/ls.tex <==
UML%


==> definitions/uml/up.tex <==
UML%


==> definitions/uml/us.tex <==
UML%


==> definitions/universe/def.tex <==
The `world' under consideration. 


==> definitions/universe/lp.tex <==
universes%


==> definitions/universe/ls.tex <==
universe%


==> definitions/universe/up.tex <==
Universes%


==> definitions/universe/us.tex <==
Universe%


==> definitions/uod/def.tex <==
That part of the world around is that is to be modelled. See also 
\DefinitionName{application-domain}{ls}.


==> definitions/uod/lp.tex <==
universes of discourse%


==> definitions/uod/ls.tex <==
universe of discourse%


==> definitions/uod/up.tex <==
Universes of discourse%


==> definitions/uod/us.tex <==
Universe of discourse%


==> definitions/usability/lp.tex <==
usabilities%


==> definitions/usability/ls.tex <==
usability%


==> definitions/usability/up.tex <==
Usabilities%


==> definitions/usability/us.tex <==
Usability%


==> definitions/view/def.tex <==
A set of \DN{model} descriptions of a \DN{domain} from the perspective of a related set of \PDN{interest} of a \DN{viewer}.



==> definitions/view/lp.tex <==
views%


==> definitions/view/ls.tex <==
view%


==> definitions/view/up.tex <==
Views%


==> definitions/view/us.tex <==
View%


==> definitions/view/view/def.tex <==
A set of \DN{model} descriptions of a \DN{domain} from the perspective of a related set of \PDN{interest} of a \DN{viewer}.



==> definitions/view/view/lp.tex <==
views%


==> definitions/view/view/ls.tex <==
view%


==> definitions/view/view/up.tex <==
Views%


==> definitions/view/view/us.tex <==
View%


==> definitions/viewer/def.tex <==
An \DN{actor} perceiving and conceiving (part of) a \DN{domain}.


==> definitions/viewer/lp.tex <==
viewers%


==> definitions/viewer/ls.tex <==
viewer%


==> definitions/viewer/up.tex <==
Viewers%


==> definitions/viewer/us.tex <==
Viewer%


==> definitions/viewing-cell/lp.tex <==
viewing cells%


==> definitions/viewing-cell/ls.tex <==
viewing cell%


==> definitions/viewing-cell/up.tex <==
Viewing cells%


==> definitions/viewing-cell/us.tex <==
Viewing cell%


==> definitions/viewing-framework/lp.tex <==
viewing frameworks%


==> definitions/viewing-framework/ls.tex <==
viewing framework%


==> definitions/viewing-framework/up.tex <==
Viewing frameworks%


==> definitions/viewing-framework/us.tex <==
Viewing framework%


==> definitions/viewing-method/def.tex <==
The \DN{method} by means of which a \DN{view} is constructed from \PDN{model}. 
A viewing \DN{method} will typically make use of modeling \PDN{method} for the
creation of these \PDN{model}.


==> definitions/viewing-method/lp.tex <==
viewing methods%


==> definitions/viewing-method/ls.tex <==
viewing method%


==> definitions/viewing-method/up.tex <==
Viewing methods%


==> definitions/viewing-method/us.tex <==
Viewing method%


==> definitions/viewing-method/viewing-method/def.tex <==
The \DN{method} by means of which a \DN{view} is constructed from \PDN{model}. 
A viewing \DN{method} will typically make use of modeling \PDN{method} for the
creation of these \PDN{model}.


==> definitions/viewing-method/viewing-method/lp.tex <==
viewing methods%


==> definitions/viewing-method/viewing-method/ls.tex <==
viewing method%


==> definitions/viewing-method/viewing-method/up.tex <==
Viewing methods%


==> definitions/viewing-method/viewing-method/us.tex <==
Viewing method%


==> definitions/viewpoint/lp.tex <==
viewpoints%


==> definitions/viewpoint/ls.tex <==
viewpoint%


==> definitions/viewpoint/up.tex <==
Viewpoints%


==> definitions/viewpoint/us.tex <==
Viewpoint%


==> definitions/viewpoint/viewpoint/def.tex <==
A combination of a \DN{viewing method} and a \DN{perspective} framework.


==> definitions/viewpoint/viewpoint/lp.tex <==
viewpoints%


==> definitions/viewpoint/viewpoint/ls.tex <==
viewpoint%


==> definitions/viewpoint/viewpoint/up.tex <==
Viewpoints%


==> definitions/viewpoint/viewpoint/us.tex <==
Viewpoint%


==> definitions/way-of-communicating/def.tex <==
describes how the abstract concepts from the \DN{way-of-modeling} 
are communicated to human beings, for example in terms of a
textual or a graphical notation.

The way of communicating essentially forms the bridge between the
way of modeling and the \DN{way-of-working}, it matches the abstract
concepts of the way of modeling to the pragmatic needs of the 
way of working.

Note that it may very well be the case that different \PDN{modeling-technique} 
are based on the same \DN{way-of-modeling}, yet use different notations.



==> definitions/way-of-communicating/lp.tex <==
way of communicating%


==> definitions/way-of-communicating/ls.tex <==
way of communicating%


==> definitions/way-of-communicating/up.tex <==
Way of communicating%


==> definitions/way-of-communicating/us.tex <==
Way of communicating%


==> definitions/way-of-conceiving/lp.tex <==
way of conceiving%


==> definitions/way-of-conceiving/ls.tex <==
way of conceiving%


==> definitions/way-of-conceiving/up.tex <==
Way of conceiving%


==> definitions/way-of-conceiving/us.tex <==
Way of conceiving%


==> definitions/way-of-controlling/def.tex <==
The managerial aspects of system engineering.  It includes such aspects as
human resource management, quality and progress control, and evaluation of
plans, i.e.\ overall project management and governance (see
\cite{1984-Kensing-MethodEvaluation, 1988-Sol-InfSystDev}).



==> definitions/way-of-controlling/lp.tex <==
way of controlling%


==> definitions/way-of-controlling/ls.tex <==
way of controlling%


==> definitions/way-of-controlling/up.tex <==
Way of controlling%


==> definitions/way-of-controlling/us.tex <==
Way of controlling%


==> definitions/way-of-delivering/def.tex <==
The languages, conventions and documentation standards used in producing
deliverables during system engineering.


==> definitions/way-of-delivering/lp.tex <==
ways of delivering%


==> definitions/way-of-delivering/ls.tex <==
way of delivering%


==> definitions/way-of-delivering/up.tex <==
Ways of delivering%


==> definitions/way-of-delivering/us.tex <==
Way of delivering%


==> definitions/way-of-delivering/way-of-delivering/def.tex <==
The languages, conventions and documentation standards used in producing
deliverables during system engineering.


==> definitions/way-of-delivering/way-of-delivering/lp.tex <==
ways of delivering%


==> definitions/way-of-delivering/way-of-delivering/ls.tex <==
way of delivering%


==> definitions/way-of-delivering/way-of-delivering/up.tex <==
Ways of delivering%


==> definitions/way-of-delivering/way-of-delivering/us.tex <==
Way of delivering%


==> definitions/way-of-describing/lp.tex <==
way of describing%


==> definitions/way-of-describing/ls.tex <==
way of describing%


==> definitions/way-of-describing/up.tex <==
Way of describing%


==> definitions/way-of-describing/us.tex <==
Way of describing%


==> definitions/way-of-learning/def.tex <==
The process and measures that enable continuous improvement of consecutive 
executions of the method. It should provide answers to questions such as: 
\emph{How can we learn from past experiences?}
\emph{How can the method be refined to reflect new experiences?}


==> definitions/way-of-learning/lp.tex <==
ways of learning%


==> definitions/way-of-learning/ls.tex <==
way of learning%


==> definitions/way-of-learning/up.tex <==
Ways of learning%


==> definitions/way-of-learning/us.tex <==
Way of learning%


==> definitions/way-of-learning/way-of-learning/def.tex <==
The process and measures that enable continuous improvement of consecutive 
executions of the method. It should provide answers to questions such as: 
\emph{How can we learn from past experiences?}
\emph{How can the method be refined to reflect new experiences?}


==> definitions/way-of-learning/way-of-learning/lp.tex <==
ways of learning%


==> definitions/way-of-learning/way-of-learning/ls.tex <==
way of learning%


==> definitions/way-of-learning/way-of-learning/up.tex <==
Ways of learning%


==> definitions/way-of-learning/way-of-learning/us.tex <==
Way of learning%


==> definitions/way-of-modeling/lp.tex <==
way of modeling%


==> definitions/way-of-modeling/ls.tex <==
way of modeling%


==> definitions/way-of-modeling/up.tex <==
Way of modeling%


==> definitions/way-of-modeling/us.tex <==
Way of modeling%


==> definitions/way-of-supporting/def.tex <==
The support to system development that is offered by (possibly automated)
tools.  In general, a way of supporting is supplied in the form of some
computerized tool (see for instance \cite{1989-McClure-CASE}).


==> definitions/way-of-supporting/lp.tex <==
way of supporting%


==> definitions/way-of-supporting/ls.tex <==
way of supporting%


==> definitions/way-of-supporting/up.tex <==
Way of supporting%


==> definitions/way-of-supporting/us.tex <==
Way of supporting%


==> definitions/way-of-thinking/lp.tex <==
way of thinking%


==> definitions/way-of-thinking/ls.tex <==
way of thinking%


==> definitions/way-of-thinking/up.tex <==
Way of thinking%


==> definitions/way-of-thinking/us.tex <==
Way of thinking%


==> definitions/way-of-using/def.tex <==
Identification of heuristics that:
\begin{itemize}
   \item define situations, classes of \PDN{viewer} and \PDN{interest}, for
   which a given \DN{viewpoint} is most suitable,
   \item provide guidance in tuning a given \DN{viewpoint} to specific situations, 
   classes of \PDN{viewer} and their \PDN{interest} at hand.

   For example, in terms of the set of modelling concepts to be used, effective
   notations, visualisations, etc.
\end{itemize}


==> definitions/way-of-using/lp.tex <==
way of using%


==> definitions/way-of-using/ls.tex <==
way of using%


==> definitions/way-of-using/up.tex <==
Way of using%


==> definitions/way-of-using/us.tex <==
Way of using%


==> definitions/way-of-working/lp.tex <==
way of working%


==> definitions/way-of-working/ls.tex <==
way of working%


==> definitions/way-of-working/up.tex <==
Way of working%


==> definitions/way-of-working/us.tex <==
Way of working%


==> definitions/weak-identification/def.tex <==
A sufficient condition to be able to uniquely identify objects and 
things, stating that no two objects or things have the same properties.


==> definitions/weak-identification/lp.tex <==
weak identification%


==> definitions/weak-identification/ls.tex <==
weak identification%


==> definitions/weak-identification/up.tex <==
Weak identification%


==> definitions/weak-identification/us.tex <==
Weak identification%


==> definitions/work-system-engineering/100-percent-principle/def.tex <==
The \DN{information-grammar} should describe \emph{precisely all} conceptual aspects. 

==> definitions/work-system-engineering/100-percent-principle/lp.tex <==
100\% Principle% 

==> definitions/work-system-engineering/100-percent-principle/ls.tex <==
100\% Principle% 

==> definitions/work-system-engineering/100-percent-principle/up.tex <==
100\% Principle% 

==> definitions/work-system-engineering/100-percent-principle/us.tex <==
100\% Principle% 

==> definitions/work-system-engineering/WSML/def.tex <==
Abbreviation for work system modeling library. A library of methodical
knowledge pertaining to the \DN{modeling} of \PDN{work-system}.


==> definitions/work-system-engineering/WSML/lp.tex <==
WSMLs%


==> definitions/work-system-engineering/WSML/ls.tex <==
WSML%


==> definitions/work-system-engineering/WSML/up.tex <==
WSMLs%


==> definitions/work-system-engineering/WSML/us.tex <==
WSML%


==> definitions/work-system-engineering/abstraction/def.tex <==
Omitting unessential details.


==> definitions/work-system-engineering/abstraction/lp.tex <==
abstractions% 

==> definitions/work-system-engineering/abstraction/ls.tex <==
abstraction% 

==> definitions/work-system-engineering/abstraction/up.tex <==
Abstractions% 

==> definitions/work-system-engineering/abstraction/us.tex <==
Abstraction% 

==> definitions/work-system-engineering/action-oriented/def.tex <==
The action-oriented approach interprets sentences as events occurring in the \DN{uod}. This approach is when the operations on the data are dominant.
See also \DN{fact-oriented}. 

==> definitions/work-system-engineering/action-oriented/lp.tex <==
action oriented% 

==> definitions/work-system-engineering/action-oriented/ls.tex <==
action oriented% 

==> definitions/work-system-engineering/action-oriented/up.tex <==
Action oriented% 

==> definitions/work-system-engineering/action-oriented/us.tex <==
Action oriented% 

==> definitions/work-system-engineering/active-system/def.tex <==
A special kind of \DN{system} that is conceived of as begin able to change
parts of the \DN{universe}.


==> definitions/work-system-engineering/active-system/lp.tex <==
active systems%


==> definitions/work-system-engineering/active-system/ls.tex <==
active system%


==> definitions/work-system-engineering/active-system/up.tex <==
Active systems%


==> definitions/work-system-engineering/active-system/us.tex <==
Active system%


==> definitions/work-system-engineering/activity-participation/def.tex <==
A \DN{system-link} between a \DN{system-activity} and one of its
\DN{actor}.


==> definitions/work-system-engineering/activity-participation/lp.tex <==
activity participations%


==> definitions/work-system-engineering/activity-participation/ls.tex <==
activity participation%


==> definitions/work-system-engineering/activity-participation/up.tex <==
Activity participations%


==> definitions/work-system-engineering/activity-participation/us.tex <==
Activity participation%


==> definitions/work-system-engineering/actor/def.tex <==
A \DN{system-element} that is conceived of as having some involvement in a
\DN{system-activity}. This involvement is a special kind of
\DN{system-link}, referred to as an \DN{activity-participation}.


==> definitions/work-system-engineering/actor/lp.tex <==
actors%


==> definitions/work-system-engineering/actor/ls.tex <==
actor%


==> definitions/work-system-engineering/actor/up.tex <==
Actors%


==> definitions/work-system-engineering/actor/us.tex <==
Actor%


==> definitions/work-system-engineering/agens/def.tex <==
The role in a sentence that most commonly is associated with the grammatical subject. 

==> definitions/work-system-engineering/agens/lp.tex <==
agens% 

==> definitions/work-system-engineering/agens/ls.tex <==
agens% 

==> definitions/work-system-engineering/agens/up.tex <==
Agens% 

==> definitions/work-system-engineering/agens/us.tex <==
Agens% 

==> definitions/work-system-engineering/alignment/def.tex <==
A \DN{system} $S_1$ is aligned to a system $S_2$ if, and only if, system $S_1$ meets {\em all} \PDN{requirement} posed by $S_2$ on $S_1$.

This alignment may be strived for at different levels of refinement of a system design.


==> definitions/work-system-engineering/alignment/lp.tex <==
alignment%


==> definitions/work-system-engineering/alignment/ls.tex <==
alignment%


==> definitions/work-system-engineering/alignment/up.tex <==
Alignment%


==> definitions/work-system-engineering/alignment/us.tex <==
Alignment%


==> definitions/work-system-engineering/application-domain/def.tex <==
That part of the world around is that is to be modelled in the context of the development of some application. See also \DN{uod}. 

==> definitions/work-system-engineering/application-domain/lp.tex <==
application domains% 

==> definitions/work-system-engineering/application-domain/ls.tex <==
application domains% 

==> definitions/work-system-engineering/application-domain/up.tex <==
Application domains% 

==> definitions/work-system-engineering/application-domain/us.tex <==
Application domain% 

==> definitions/work-system-engineering/approach/def.tex <==
\Synonym{way-of-working}


==> definitions/work-system-engineering/approach/lp.tex <==
approaches%


==> definitions/work-system-engineering/approach/ls.tex <==
approach%


==> definitions/work-system-engineering/approach/up.tex <==
Approaches%


==> definitions/work-system-engineering/approach/us.tex <==
Approach%


==> definitions/work-system-engineering/architecting/def.tex <==
The processes which tie \DN{definition}, \DN{design} and \DN{deployment} and
to the explicit and implicit needs, desires and requirements
of the usage context. Issues such as: business/IT alignment, stakeholders,
limiting design freedom, negotiation between stakeholders, enterprise
architectures, stakeholder communication, and outsourcing, typify these
processes. 


==> definitions/work-system-engineering/architecting/lp.tex <==
architecting%


==> definitions/work-system-engineering/architecting/ls.tex <==
architecting%


==> definitions/work-system-engineering/architecting/up.tex <==
Architecting%


==> definitions/work-system-engineering/architecting/us.tex <==
Architecting%


==> definitions/work-system-engineering/architectural-description/def.tex <==
A \DN{system-description} documenting/describing an \DN{architecture}.


==> definitions/work-system-engineering/architectural-description/lp.tex <==
architectural descriptions%


==> definitions/work-system-engineering/architectural-description/ls.tex <==
architectural description%


==> definitions/work-system-engineering/architectural-description/up.tex <==
Architectural descriptions%


==> definitions/work-system-engineering/architectural-description/us.tex <==
Architectural description%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/def.tex <==
\UDN{information-system-engineering}, using \DN{architecture} as a means to
\begin{itemize}
   \item guide \& control the design and evolution of the \DN{information-system},
   \item evaluate \& compare different information system alternatives, 
   \item negotiate the \PDN{concern} of the information system's \PDN{stakeholder},
\end{itemize}
with the aim of optimising the \DN{alignment} of the resulting
information system to its relevant, technological, organisation and human context (systems).


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/lp.tex <==
architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/ls.tex <==
architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/up.tex <==
Architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/us.tex <==
Architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-principle/def.tex <==
A \DN{design-principle} which is used to direct the design/architecting of
an \DN{architecture}.


==> definitions/work-system-engineering/architecture-principle/lp.tex <==
architecture principles%


==> definitions/work-system-engineering/architecture-principle/ls.tex <==
architecture principle%


==> definitions/work-system-engineering/architecture-principle/up.tex <==
Architecture principles%


==> definitions/work-system-engineering/architecture-principle/us.tex <==
Architecture principle%


==> definitions/work-system-engineering/architecture/def.tex <==
A \DN{model} of which the \DN{system-description}, the so-called
\DN{architectural-description}, is used during \DN{system-engineering} to:
    \begin{itemize}
      \item express the fundamental organization of the \DN{system-domain} in 
    terms of \PDN{component}, their relationships to each other and 
    to the \DN{environment} and 
      \item the principles guiding its evolution and design,
    \end{itemize}
    and which's explicit intend is to be used as a means:
    \begin{itemize}
      \item of communication \& negotiation among stakeholders,
      \item to evaluate and compare design alternatives,
      \item to plan, manage, and execute further system development,
      \item to verify the compliance of a system implementation's.
    \end{itemize}
  


==> definitions/work-system-engineering/architecture/lp.tex <==
architectures%


==> definitions/work-system-engineering/architecture/ls.tex <==
architecture%


==> definitions/work-system-engineering/architecture/up.tex <==
Architectures%


==> definitions/work-system-engineering/architecture/us.tex <==
Architecture%


==> definitions/work-system-engineering/aspect-system/def.tex <==
an aspect-system $S'$ of a \DN{system} $S$, is a \DN{sub-system}, where the set
of \PDN{model-link} in $S'$ is a proper subset of the set of the
\PDN{link} in $S$.


==> definitions/work-system-engineering/aspect-system/lp.tex <==
aspect systems%


==> definitions/work-system-engineering/aspect-system/ls.tex <==
aspect system%


==> definitions/work-system-engineering/aspect-system/up.tex <==
Aspect systems%


==> definitions/work-system-engineering/aspect-system/us.tex <==
Aspect system%


==> definitions/work-system-engineering/atomic-viewpoint/def.tex <==
A \DN{viewpoint} which is not decomposed into smaller \PDN{viewpoint}. An
\DN{atomic-viewpoint} is required to have a one-on-one correspondence to a
\DN{way-of-modeling}/\DN{technique} that should be used to create \PDN{model}
conforming to this \DN{viewpoint}.


==> definitions/work-system-engineering/atomic-viewpoint/lp.tex <==
atomic viewpoints%


==> definitions/work-system-engineering/atomic-viewpoint/ls.tex <==
atomic viewpoint%


==> definitions/work-system-engineering/atomic-viewpoint/up.tex <==
Atomic viewpoints%


==> definitions/work-system-engineering/atomic-viewpoint/us.tex <==
Atomic viewpoint%


==> definitions/work-system-engineering/autonomous-system/def.tex <==
an \DN{open-active-system} (possibly also a \DN{responsive-system}, but not a
\DN{reactive-system}) where at least one expression is an action.  A human
being and most (if not all) \PDN{organization} can be regarded as 
\PDN{autonomous-system}.



==> definitions/work-system-engineering/autonomous-system/lp.tex <==
autonomous systems%


==> definitions/work-system-engineering/autonomous-system/ls.tex <==
autonomous system%


==> definitions/work-system-engineering/autonomous-system/up.tex <==
Autonomous systems%


==> definitions/work-system-engineering/autonomous-system/us.tex <==
Autonomous system%


==> definitions/work-system-engineering/characterization-dimension/def.tex <==
A set of (possibly ordered) values by which an artefact may be characterized.


==> definitions/work-system-engineering/characterization-dimension/lp.tex <==
characterization dimensions%


==> definitions/work-system-engineering/characterization-dimension/ls.tex <==
characterization dimension%


==> definitions/work-system-engineering/characterization-dimension/up.tex <==
Characterization dimensions%


==> definitions/work-system-engineering/characterization-dimension/us.tex <==
Characterization dimension%


==> definitions/work-system-engineering/characterization-property/def.tex <==
A specific value from a \DN{characterization-dimension} that an artefact may
exhibit. 


==> definitions/work-system-engineering/characterization-property/lp.tex <==
characterization properties%


==> definitions/work-system-engineering/characterization-property/ls.tex <==
characterization property%


==> definitions/work-system-engineering/characterization-property/up.tex <==
Characterization properties%


==> definitions/work-system-engineering/characterization-property/us.tex <==
Characterization property%


==> definitions/work-system-engineering/closed-world-assumption/def.tex <==
All facts not stored in an \DN{information-system} are assumed to be false.
Not that this requires facts with \DN{complete-knowledge}. 

==> definitions/work-system-engineering/closed-world-assumption/lp.tex <==
closed world assumptions% 

==> definitions/work-system-engineering/closed-world-assumption/ls.tex <==
closed world assumption% 

==> definitions/work-system-engineering/closed-world-assumption/up.tex <==
Closed world assumptions% 

==> definitions/work-system-engineering/closed-world-assumption/us.tex <==
Closed world assumption% 

==> definitions/work-system-engineering/communication/def.tex <==
An exchange of \PDN{message}, i.e.\ a sequence of mutual and alternating
message transfers between at least two \PDN{human-actor}, called communication
partners, whereby these \PDN{message} represent some \DN{knowledge} and are
expressed in languages understood by all communication partners, and whereby
some amount of \DN{knowledge} about the domain of communication and about the
action context and the goal of the communication is made present in all
communication partners.



==> definitions/work-system-engineering/communication/lp.tex <==
communications%


==> definitions/work-system-engineering/communication/ls.tex <==
communication%


==> definitions/work-system-engineering/communication/up.tex <==
Communications%


==> definitions/work-system-engineering/communication/us.tex <==
Communication%


==> definitions/work-system-engineering/complete-knowledge/def.tex <==
The value \emph{undefined} is not allowed.


==> definitions/work-system-engineering/complete-knowledge/lp.tex <==
complete knowledge% 

==> definitions/work-system-engineering/complete-knowledge/ls.tex <==
complete knowledge% 

==> definitions/work-system-engineering/complete-knowledge/up.tex <==
Complete knowledge% 

==> definitions/work-system-engineering/complete-knowledge/us.tex <==
Complete knowledge% 

==> definitions/work-system-engineering/component-system/def.tex <==
A component-system $S'$ of a \DN{system} $S$, is a \DN{sub-system},  where the
set of \PDN{model-concept} in $S'$ is a proper subset of the set of entities in
$S$.


==> definitions/work-system-engineering/component-system/lp.tex <==
component systems%


==> definitions/work-system-engineering/component-system/ls.tex <==
component system%


==> definitions/work-system-engineering/component-system/up.tex <==
Component systems%


==> definitions/work-system-engineering/component-system/us.tex <==
Component system%


==> definitions/work-system-engineering/component/def.tex <==
\AbbreviationOf{component-system}



==> definitions/work-system-engineering/component/lp.tex <==
components%


==> definitions/work-system-engineering/component/ls.tex <==
component%


==> definitions/work-system-engineering/component/up.tex <==
Components%


==> definitions/work-system-engineering/component/us.tex <==
Component%


==> definitions/work-system-engineering/computerized-information-system/def.tex <==
A \DN{sub-system} of an \DN{information-system}, whereby all activities within
that sub-system are performed by one or several computer(s).	


==> definitions/work-system-engineering/computerized-information-system/lp.tex <==
computerized information systems%


==> definitions/work-system-engineering/computerized-information-system/ls.tex <==
computerized information system%


==> definitions/work-system-engineering/computerized-information-system/up.tex <==
Computerized information systems%


==> definitions/work-system-engineering/computerized-information-system/us.tex <==
Computerized information system%


==> definitions/work-system-engineering/concept/def.tex <==
Any \DN{element} from a \DN{conception} that is not a \DN{link}.


==> definitions/work-system-engineering/concept/lp.tex <==
concepts%


==> definitions/work-system-engineering/concept/ls.tex <==
concept%


==> definitions/work-system-engineering/concept/up.tex <==
Concepts%


==> definitions/work-system-engineering/concept/us.tex <==
Concept%


==> definitions/work-system-engineering/conception-evolution/def.tex <==
The evolution of a \DN{conception}.


==> definitions/work-system-engineering/conception-evolution/lp.tex <==
conception evolutions%


==> definitions/work-system-engineering/conception-evolution/ls.tex <==
conception evolution%


==> definitions/work-system-engineering/conception-evolution/up.tex <==
Conception evolutions%


==> definitions/work-system-engineering/conception-evolution/us.tex <==
Conception evolution%


==> definitions/work-system-engineering/conception/def.tex <==
That what results, in the mind of a \DN{viewer}, when they interpret a
\DN{perception} of a \DN{domain}.


==> definitions/work-system-engineering/conception/lp.tex <==
conceptions%


==> definitions/work-system-engineering/conception/ls.tex <==
conception%


==> definitions/work-system-engineering/conception/up.tex <==
Conceptions%


==> definitions/work-system-engineering/conception/us.tex <==
Conception%


==> definitions/work-system-engineering/conceptualization-principle/def.tex <==
The \DN{information-grammar} should not describe any does \emph{not} provide any realization (implementation) aspect. 

==> definitions/work-system-engineering/conceptualization-principle/lp.tex <==
Conceptualization principle% 

==> definitions/work-system-engineering/conceptualization-principle/ls.tex <==
conceptualization principle% 

==> definitions/work-system-engineering/conceptualization-principle/up.tex <==
Conceptualization principle% 

==> definitions/work-system-engineering/conceptualization-principle/us.tex <==
Conceptualization principle% 

==> definitions/work-system-engineering/def.tex <==
A process aimed at adapting a \DefinitionName{work-system}{ls} to 
(possibly implicit and informal) needs, using limited means. These 
processes involving the execution of four sub-processes: 
\DefinitionName{definition-process}{ls}, 
\DefinitionName{design-process}{ls}, 
\DefinitionName{construction-process}{ls} and 
\DefinitionName{deployment-process}{ls}. Processes that may be executed 
sequentially, incrementally, interleaved, or in parallel.


==> definitions/work-system-engineering/lp.tex <==
work system engineering%


==> definitions/work-system-engineering/ls.tex <==
work system engineering%


==> definitions/work-system-engineering/up.tex <==
Work system engineering%


==> definitions/work-system-engineering/us.tex <==
Work system engineering%


==> definitions/work-system/lp.tex <==
work systems%


==> definitions/work-system/ls.tex <==
work system%


==> definitions/work-system/up.tex <==
Work systems%


==> definitions/work-system/us.tex <==
Work system%


==> generate <==
#!/bin/bash

# genbib lives here:
PATH=~erikp/bin:$PATH

BIBTEX=bibtex
GENBIB=genbib
MAKEINDEX=makeindex
CITATIONS=Citations
CONCEPTS=Concepts

function Tell () {
  echo
  echo "--------------------------------------------------------------------------------"
  echo "   $1"
  echo "--------------------------------------------------------------------------------"
  echo
}

function LaTeX () {
  Tell "Running LaTeX"

  $LATEX $1

  Tell "Finished running LaTeX"
}

function ListKeysFromAux () {
  cat *.aux \
  | egrep "^.citation" \
  | sed -e "s/.*{//" \
  | sed -e "s/,/ /g" \
  | sed -e "s/}.*//" \
  | sort -u
}

function GenBib () {
  Tell "Running GenBib"

  if [ ! -e new.bib ]; then
     echo > new.bib
  fi
  if [ ! -e all.bib ]; then
     echo > all.bib
  fi

  mv all.bib all.bib-bak
  $GENBIB
 
  if [ "`grep -c "@" all.bib`" == "0"  ]; then 
     mv all.bib-bak all.bib
  fi

  Tell "Finished running GenBib"
}

function TryBibTeX () {
  # This wrapper for bibtex tries to avoid generating an empty bbl file.

  if [ -f $1.aux ]; then
    $BIBTEX $1
    if [ `grep -c bibitem $1.bbl` = 0 ]; then
      rm $1.bbl
    fi
  fi
}

function BibTeX () {
  Tell "Running BibTeX"

  rm $1.bbl 2> /dev/null
  TryBibTeX $1

  BIBDATA="` cat $1.aux | grep "bibdata" `"
  BIBSTYLE="`cat $1.aux | grep "bibstyle"`"

  # For each of the chapters, we should run BibTeX seperately. This is needed
  # for the bibliography of chapters.
  if [ -f $1.chp ]; then
    for f in `cat $1.chp`; do
      rm $f.bbl $f.mbl 2> /dev/null
   
      cat $f.aux     >  tmp.aux
      echo $BIBDATA  >> tmp.aux
      echo $BIBSTYLE >> tmp.aux
   
      TryBibTeX tmp
      if [ -f tmp.bbl ]; then
        mv tmp.bbl $f.bbl

        # Get the longest bibtex label:
	cat $f.bbl \
	| grep begin \
	| grep thebiblio \
	| sed -e "s/.*graphy}{//" \
	| sed -e "s/}$//" \
	> $f.mbl
      fi
   
      rm tmp.*
    done
  fi
  
  Tell "Finished running BibTeX"
}

function Dictionary () {
  Tell "Producing dictionary"
  if [ -s "$1.dic" ]; then
    echo "\begin{Definitions}" >  $1.dct
    cat $1.dic | sort -u       >> $1.dct
    echo "\end{Definitions}"   >> $1.dct
  else
    echo                       >  $1.dct 
  fi
  Tell "Finished producing dictionary"
}

function SymbolList () {
  Tell "Producing symbol list"
  if [ -s "$1.sym" ]; then 
    echo "\begin{Symbols}" >  $1.smb
    cat $1.sym | sort -u   >> $1.smb
    echo "\end{Symbols}"   >> $1.smb
  else
    echo                   >  $1.smb
  fi
  Tell "Finished producing symbol list"
}

function ListCitations () {
  cat *.aux  \
  | grep "\citation" \
  | sed -e "s/.citation{//" \
  | sed -e "s/}.*//" \
  | sort -u
}

function GetCitation () {
   echo -n .

   # First retreive a plain LaTeX version of the BibTeX entry
   echo "\citation{$1}"                 >  tmp.aux
   echo "\bibstyle{../style/plain.bst}" >> tmp.aux
   echo "\bibdata{new,all}"             >> tmp.aux
   $BIBTEX tmp > /dev/null 2> /dev/null
  
   # Remove any unnecessary/unwanted BibTeX related LaTeX commands:
   cat tmp.bbl \
   | sed -e "s/\\\\newblock//" \
   | sed -e "s/\\\\begin.*//" \
   | sed -e "s/\\\\end.*//" \
   | sed -e "s/\\\\bibitem.*//" \
   | sed -e "s/$/ %/" \
   | sed -e "s/^ *//" \
   > $CITATIONS/$1.tex

   # Now we need to retrieve the author list of the entry.
   echo "\citation{$1}"                   >  tmp.aux
   echo "\bibstyle{../style/authors.bst}" >> tmp.aux
   echo "\bibdata{new,all}"               >> tmp.aux
   $BIBTEX tmp > /dev/null 2> /dev/null

   # Split-off the authors into separate fields, and remove unwanted
   # characters.
   words="`cat tmp.bbl \
          | sed -e "s/~/ /g" \
          | sed -e "s/{//g" \
          | sed -e "s/}//g"`"

   rm $CITATIONS/$1.author 2> /dev/null
   author=""
   for word in $words; do
     echo -n .
     if [ "$word" == "[and]" ]; then
       if [ -n "$author" ]; then
         if [ "$author" != "others" ]; then
            echo "\authorindex{$author}%" >> $CITATIONS/$1.author
            author=""
	 fi
       fi
     else
       if [ -n "$author" ]; then
         author="$author $word"
       else
         author="$word"
       fi
     fi
   done

   rm tmp.*
}

function GetCitations () {
  Tell "Producing citations"

  rm -rf $CITATIONS 2> /dev/null
  mkdir -p $CITATIONS

  for c in `ListCitations`; do
    GetCitation $c Citations 
  done
  echo

  Tell "Finished producing citations"
}

function AuthorIndex () {
  if [ -f $1-au.idx ]; then
    Tell "Building author index"

    echo 'headings_flag 1'                  >  $$
    echo 'heading_prefix "{\\bf "'          >> $$
    echo 'heading_suffix "} \\nopagebreak"' >> $$
    $MAKEINDEX $1-au -s $$
    rm $$

    Tell "Finished building author index"
 else
    rm $1-au.ind
 fi
}

function SubjectIndex () {
  if [ -f $1.idx ]; then
    Tell "Building subject index"

    echo 'headings_flag 1'                  >  $$
    echo 'heading_prefix "{\\bf "'          >> $$
    echo 'heading_suffix "} \\nopagebreak"' >> $$
    $MAKEINDEX $1 -s $$
    rm $$

    Tell "Finished building subject index"
  else
    rm $1.ind
  fi
}

function GetConcepts () {
  if [ -f $1-sub.idx ]; then
    Tell "Producing concepts"
    rm -rf $CONCEPTS 2> /dev/null
    mkdir -p $CONCEPTS

    for c in `cat $1-sub.idx | sort -u`; do
      echo -n .
      if [ -e "../definitions/$c/ls.tex" ]; then
         concept="`cat ../definitions/$c/ls.tex \
                  | sed -e "s/%.*//"`"
      else
         concept="`cat ./definitions/$c/ls.tex \
                  | sed -e "s/%.*//"`"
      fi
      echo "\\index{$concept|DefinitionNrFont}%" > $CONCEPTS/$c.def
      echo "\\index{$concept|DictionaryNrFont}%" > $CONCEPTS/$c.dic
      echo "\\index{$concept|OccurrenceNrFont}%" > $CONCEPTS/$c.occ
    done
    echo

    Tell "Finished producing concepts"
  fi
}

function MakePDF () {
  if [ "$MAKEPDF" != "" ]; then
    Tell "Producing PDF version"

    $MAKEPDF $1
  fi
}

function DictionarySize () {
  cat $1.dct 2> /dev/null \
  | sort -u \
  | wc -l
}

function TryPrep () {
  if [ -n "$PREP" ]; then
     ./$PREP $1
  fi
}

function Generate () {
  rm *.aux *.dct *.dic *.idx *.ind *.log 2> /dev/null

  TryPrep      $1

  # Since definitions of the terms used may refer to yet other terms with a
  # definition, we need to do a "fixed-point" run:
  OLDDICTSIZE="-1"
  NEWDICTSIZE="0"
  while [ "$OLDDICTSIZE" != "$NEWDICTSIZE" ]; do
    OLDDICTSIZE=$NEWDICTSIZE
      LaTeX       $1
      Dictionary  $1
    NEWDICTSIZE="`DictionarySize $1`"
  done

  GetConcepts  $1
  GenBib 
  BibTeX       $1
  GetCitations $1
  SymbolList   $1

  LaTeX        $1
  LaTeX        $1
 
  AuthorIndex  $1
  SubjectIndex $1

  LaTeX        $1
  LaTeX        $1
  MakePDF      $1
}

# Initialise parameters 
FILE=
PREP=
LATEX=
MAKEPDF=
PUBLISH=

source ./generate.info

Generate $FILE

if [ `echo $0 | egrep -c "publish$"` -ge 1 ]; then
   echo 
   echo Copying $FILE.pdf to $PUBLISH
   cp $FILE.pdf $PUBLISH
fi


==> images/jpgtoall <==
#!/bin/bash
function Convert () {
   FILE="`echo $1 | sed -e "s/.jpg$//"`"

   if [ -e $FILE.jpg ]; then
      echo Conversions for \"$FILE\":

      echo -n "  "
      jpegtopnm $FILE.jpg             2> /dev/null \
      | pnmtops -noturn -nosetpage 2> /dev/null > $FILE.eps
      echo "$FILE.jpg --> $FILE.eps"

      echo -n "  "
      echo "$FILE.jpg --> $FILE.pdf"
      epstopdf $FILE.eps

      echo
   else
      echo Can not find: $FILE.jpg
   fi
}

if [ "$1" == "" ]; then
   for f in *.jpg; do 
       Convert $f
   done
else
   Convert $1
fi


==> publish <==
#!/bin/bash

# genbib lives here:
PATH=~erikp/bin:$PATH

BIBTEX=bibtex
GENBIB=genbib
MAKEINDEX=makeindex
CITATIONS=Citations
CONCEPTS=Concepts

function Tell () {
  echo
  echo "--------------------------------------------------------------------------------"
  echo "   $1"
  echo "--------------------------------------------------------------------------------"
  echo
}

function LaTeX () {
  Tell "Running LaTeX"

  $LATEX $1

  Tell "Finished running LaTeX"
}

function ListKeysFromAux () {
  cat *.aux \
  | egrep "^.citation" \
  | sed -e "s/.*{//" \
  | sed -e "s/,/ /g" \
  | sed -e "s/}.*//" \
  | sort -u
}

function GenBib () {
  Tell "Running GenBib"

  if [ ! -e new.bib ]; then
     echo > new.bib
  fi
  if [ ! -e all.bib ]; then
     echo > all.bib
  fi

  mv all.bib all.bib-bak
  $GENBIB
 
  if [ "`grep -c "@" all.bib`" == "0"  ]; then 
     mv all.bib-bak all.bib
  fi

  Tell "Finished running GenBib"
}

function TryBibTeX () {
  # This wrapper for bibtex tries to avoid generating an empty bbl file.

  if [ -f $1.aux ]; then
    $BIBTEX $1
    if [ `grep -c bibitem $1.bbl` = 0 ]; then
      rm $1.bbl
    fi
  fi
}

function BibTeX () {
  Tell "Running BibTeX"

  rm $1.bbl 2> /dev/null
  TryBibTeX $1

  BIBDATA="` cat $1.aux | grep "bibdata" `"
  BIBSTYLE="`cat $1.aux | grep "bibstyle"`"

  # For each of the chapters, we should run BibTeX seperately. This is needed
  # for the bibliography of chapters.
  if [ -f $1.chp ]; then
    for f in `cat $1.chp`; do
      rm $f.bbl $f.mbl 2> /dev/null
   
      cat $f.aux     >  tmp.aux
      echo $BIBDATA  >> tmp.aux
      echo $BIBSTYLE >> tmp.aux
   
      TryBibTeX tmp
      if [ -f tmp.bbl ]; then
        mv tmp.bbl $f.bbl

        # Get the longest bibtex label:
	cat $f.bbl \
	| grep begin \
	| grep thebiblio \
	| sed -e "s/.*graphy}{//" \
	| sed -e "s/}$//" \
	> $f.mbl
      fi
   
      rm tmp.*
    done
  fi
  
  Tell "Finished running BibTeX"
}

function Dictionary () {
  Tell "Producing dictionary"
  if [ -s "$1.dic" ]; then
    echo "\begin{Definitions}" >  $1.dct
    cat $1.dic | sort -u       >> $1.dct
    echo "\end{Definitions}"   >> $1.dct
  else
    echo                       >  $1.dct 
  fi
  Tell "Finished producing dictionary"
}

function SymbolList () {
  Tell "Producing symbol list"
  if [ -s "$1.sym" ]; then 
    echo "\begin{Symbols}" >  $1.smb
    cat $1.sym | sort -u   >> $1.smb
    echo "\end{Symbols}"   >> $1.smb
  else
    echo                   >  $1.smb
  fi
  Tell "Finished producing symbol list"
}

function ListCitations () {
  cat *.aux  \
  | grep "\citation" \
  | sed -e "s/.citation{//" \
  | sed -e "s/}.*//" \
  | sort -u
}

function GetCitation () {
   echo -n .

   # First retreive a plain LaTeX version of the BibTeX entry
   echo "\citation{$1}"                 >  tmp.aux
   echo "\bibstyle{../style/plain.bst}" >> tmp.aux
   echo "\bibdata{new,all}"             >> tmp.aux
   $BIBTEX tmp > /dev/null 2> /dev/null
  
   # Remove any unnecessary/unwanted BibTeX related LaTeX commands:
   cat tmp.bbl \
   | sed -e "s/\\\\newblock//" \
   | sed -e "s/\\\\begin.*//" \
   | sed -e "s/\\\\end.*//" \
   | sed -e "s/\\\\bibitem.*//" \
   | sed -e "s/$/ %/" \
   | sed -e "s/^ *//" \
   > $CITATIONS/$1.tex

   # Now we need to retrieve the author list of the entry.
   echo "\citation{$1}"                   >  tmp.aux
   echo "\bibstyle{../style/authors.bst}" >> tmp.aux
   echo "\bibdata{new,all}"               >> tmp.aux
   $BIBTEX tmp > /dev/null 2> /dev/null

   # Split-off the authors into separate fields, and remove unwanted
   # characters.
   words="`cat tmp.bbl \
          | sed -e "s/~/ /g" \
          | sed -e "s/{//g" \
          | sed -e "s/}//g"`"

   rm $CITATIONS/$1.author 2> /dev/null
   author=""
   for word in $words; do
     echo -n .
     if [ "$word" == "[and]" ]; then
       if [ -n "$author" ]; then
         if [ "$author" != "others" ]; then
            echo "\authorindex{$author}%" >> $CITATIONS/$1.author
            author=""
	 fi
       fi
     else
       if [ -n "$author" ]; then
         author="$author $word"
       else
         author="$word"
       fi
     fi
   done

   rm tmp.*
}

function GetCitations () {
  Tell "Producing citations"

  rm -rf $CITATIONS 2> /dev/null
  mkdir -p $CITATIONS

  for c in `ListCitations`; do
    GetCitation $c Citations 
  done
  echo

  Tell "Finished producing citations"
}

function AuthorIndex () {
  if [ -f $1-au.idx ]; then
    Tell "Building author index"

    echo 'headings_flag 1'                  >  $$
    echo 'heading_prefix "{\\bf "'          >> $$
    echo 'heading_suffix "} \\nopagebreak"' >> $$
    $MAKEINDEX $1-au -s $$
    rm $$

    Tell "Finished building author index"
 else
    rm $1-au.ind
 fi
}

function SubjectIndex () {
  if [ -f $1.idx ]; then
    Tell "Building subject index"

    echo 'headings_flag 1'                  >  $$
    echo 'heading_prefix "{\\bf "'          >> $$
    echo 'heading_suffix "} \\nopagebreak"' >> $$
    $MAKEINDEX $1 -s $$
    rm $$

    Tell "Finished building subject index"
  else
    rm $1.ind
  fi
}

function GetConcepts () {
  if [ -f $1-sub.idx ]; then
    Tell "Producing concepts"
    rm -rf $CONCEPTS 2> /dev/null
    mkdir -p $CONCEPTS

    for c in `cat $1-sub.idx | sort -u`; do
      echo -n .
      if [ -e "../definitions/$c/ls.tex" ]; then
         concept="`cat ../definitions/$c/ls.tex \
                  | sed -e "s/%.*//"`"
      else
         concept="`cat ./definitions/$c/ls.tex \
                  | sed -e "s/%.*//"`"
      fi
      echo "\\index{$concept|DefinitionNrFont}%" > $CONCEPTS/$c.def
      echo "\\index{$concept|DictionaryNrFont}%" > $CONCEPTS/$c.dic
      echo "\\index{$concept|OccurrenceNrFont}%" > $CONCEPTS/$c.occ
    done
    echo

    Tell "Finished producing concepts"
  fi
}

function MakePDF () {
  if [ "$MAKEPDF" != "" ]; then
    Tell "Producing PDF version"

    $MAKEPDF $1
  fi
}

function DictionarySize () {
  cat $1.dct 2> /dev/null \
  | sort -u \
  | wc -l
}

function TryPrep () {
  if [ -n "$PREP" ]; then
     ./$PREP $1
  fi
}

function Generate () {
  rm *.aux *.dct *.dic *.idx *.ind *.log 2> /dev/null

  TryPrep      $1

  # Since definitions of the terms used may refer to yet other terms with a
  # definition, we need to do a "fixed-point" run:
  OLDDICTSIZE="-1"
  NEWDICTSIZE="0"
  while [ "$OLDDICTSIZE" != "$NEWDICTSIZE" ]; do
    OLDDICTSIZE=$NEWDICTSIZE
      LaTeX       $1
      Dictionary  $1
    NEWDICTSIZE="`DictionarySize $1`"
  done

  GetConcepts  $1
  GenBib 
  BibTeX       $1
  GetCitations $1
  SymbolList   $1

  LaTeX        $1
  LaTeX        $1
 
  AuthorIndex  $1
  SubjectIndex $1

  LaTeX        $1
  LaTeX        $1
  MakePDF      $1
}

# Initialise parameters 
FILE=
PREP=
LATEX=
MAKEPDF=
PUBLISH=

source ./generate.info

Generate $FILE

if [ `echo $0 | egrep -c "publish$"` -ge 1 ]; then
   echo 
   echo Copying $FILE.pdf to $PUBLISH
   cp $FILE.pdf $PUBLISH
fi


==> series/davinci.tex <==
\nonumchapter{The \DaVinci\ Series}
\Version{30-08-05}

The subtitle of the \DaVinci\ series of lecture notes is \emph{\DaVinciSub}.
On the one hand, this series of lecture notes takes a fundamental view
(\emph{craft}) on the field information systems engineering. At the same time,
it does so with an open eye to practical experiences (the \emph{art}) gained
from information system engineering in industry.

The kinds of information systems we are interested in range from personal
information appliances to enterprise-wide information processing. Even more, we
regard an information system as a system that ``handles'' information, where
``handling'' should be interpreted in a broad fashion. The actors that do this
``handling'' can be computers, but can equally well be other ``symbol wielding
machines'', but can also be humans. The mix of humans and computers/machines in
information systems makes the field of information system engineering
particularly challenging.

The concept of ``information'' itself is very much related to the concepts of
\emph{data}, \emph{knowledge} and \emph{communication}. Based
on~\cite{1998-Lindgreen-FRISCO}, we will (throughout the \DaVinci\ series) use
the following definitions: 
\begin{Definitions}
   \DefinitionItem{data}
   \DefinitionItem{information}
   \DefinitionItem{knowledge}
   \DefinitionItem{communication}
\end{Definitions}
When referring to an information system, we therefore really refer to systems
that enable the communication/sharing of knowledge by means of the
representation (by \PDN{human-actor}), storage, processing, retrieval, and
presentation (to \PDN{human-actor}) of the underlying representations (data).
This also implies that we will treat \emph{information retrieval systems},
\emph{knowledge-based systems}, \emph{groupware systems}, etc., as special
classes of information systems.

The lecture notes in the \DaVinci\ series have been organized around four key
key processes in an information system's life-cycle:
\begin{description}
   \DefinitionItem{definition-process}
   \DefinitionItem{design-process}
   \DefinitionItem{realization-process}
   \DefinitionItem{architecting}
   \DefinitionItem{domain-modeling}
\end{description}
For each these aspects, attention will be paid to relevant theories, methods
and techniques to execute the tasks involved. When put together, these aspects
can be related as depicted in figure~\ref{davinci}.  Note that we regard
maintenance of systems as being functionality that should be designed ``into''
the system. If a system needs to be maintained, and in most cases one indeed
wants to, then the maintenance should be designed into the workings of this
system and/or its context.
\Image{7cm}{Aspects of Information Systems Engineering}{davinci}

The use of the name \DaVinci\ originates from earlier
work~\cite{1998-Proper-DaVinci} done on architecture-driven information systems
engineering. The work reported in~\cite{1998-Proper-DaVinci} was the result of
a confrontation between industrial practice and a theoretical perspective on
information systems and their evolution~\cite{1994-Proper-EvolvConcModels}. The
result was a shared vision on the architecture-driven development of
information systems by a Dutch IT consultancy firm. In this shared vision, a
foundation was laid for an integrated view on information system engineering.
At that stage, the name ``\DaVinci'' was also selected. Not as some artificial
acronym, but rather to honor an inspiring artist, scientist, inventor and
architect. To us he personifies a balance between art and engineering, between
human and technology.

After the development of the first \DaVinci\ version, a more elaborate
version~\cite{2004-Proper-DaVinci} was developed at the Radboud University
Nijmegen in the form of lecture notes associated to a course on
\emph{Architecture \& Alignment}. In this version, a more fundamental outlook
on information system development was added to complement the practical
orientation of the first version.

As a third step, we have now taken on the underlying philosophy of the first
two \DaVinci\ documents, and used this as the source of inspiration to shape an
entire line of lecture notes for a number of mutually related courses on
different aspects of information systems engineering. In making this step we
have also been able to anchor some of the fundamental research results from the
co-authors, on subjects such as information modeling~\cite{1991-Bommel-PredMod,
1991-Bommel-CSTransform, 1993-Hofstede-PSM, 1993-Hofstede-LISA-D,
1994-Proper-EvolvPSM, 1995-Brouwer-ORMKernel, 1995-Campbell-Abstraction,
1996-Proper-CDMKernel, 1995-Proper-EvolvAM, 1996-Frederiks-Logbooks,
1997-Hofstede-Grammar, 1997-Proper-Versions, 1997-Hoppenbrouwers-NLStructures,
2002-Frederiks-Infogrammars, 2004-Frederiks-InformationModeling}, information
retrieval~\cite{1990-Bruza-AssessingQuality, 1991-Bruza-Retlogic,
1991-Bruza-StratHypmed, 1996-Berger-SemRel, 1998-Wondergem-IndExprMatching,
1999-Sarbo-MeaningExtraction, 1999-Proper-Infons, 2001-Papazoglou-DigiLib,
2001-Wondergem-LogicLinguistic}, (enterprise) information
architecture~\cite{2004-Jonkers-ArchiConcepts} and information system
engineering~\cite{1999-Proper-ISPL-LSM, 2004-VeldhuijzenVanZanten-Rational}
into the core of the \DaVinci\ series.

